RT-MOT: Confidence-Aware Real-Time Scheduling Framework for Multi-Object Tracking Tasks

Different from existing MOT (Multi-Object Tracking) techniques that usually aim at improving tracking accuracy and average FPS, real-time systems such as autonomous vehicles necessitate new requirements of MOT under limited computing resources: (R1) guarantee of timely execution and (R2) high tracking accuracy. In this paper, we propose RT-MOT, a novel system design for multiple MOT tasks, which addresses R1 and R2. Focusing on multiple choices of a workload pair of detection and association, which are two main components of the tracking-by-detection approach for MOT, we tailor a measure of object confidence for RT-MOT and develop how to estimate the measure for the next frame of each MOT task. By utilizing the estimation, we make it possible to predict tracking accuracy variation according to different workload pairs to be applied to the next frame of an MOT task. Next, we develop a novel confidence-aware real-time scheduling framework, which offers an offline timing guarantee for a set of MOT tasks based on non-preemptive fixed-priority scheduling with the smallest workload pair. At run-time, the framework checks the feasibility of a priority-inversion associated with a larger workload pair, which does not compromise the timing guarantee of every task, and then chooses a feasible scenario that yields the largest tracking accuracy improvement based on the proposed prediction. Our experiment results demonstrate that RT-MOT significantly improves overall tracking accuracy by up to 1.5x, compared to existing popular tracking-by-detection approaches, while guaranteeing timely execution of all MOT tasks.

==> old.tex <==

\section{Introduction (OLD)}

\jlcmt{Flow}

- (백교수 아래 설명 참고) MOT 배경 설명, DNN-based MOT의 기본적인 구조 설명(detention, association, update, prediction).

- (백교수 아래 설명 참고) 현재 MOT 들은 주로 high accuracy and average FPS를 주로 목적으로 하고 있어 safety-critical real-time systems에 적합하지 않음. 우리는 limited resource하에서 아래를 달성하는 것이 필요함.
\begin{itemize}
    \item [O1.] timely execution of tracking should be guaranteed, and
    \item [O2.] tracking accuracy should be high, but differentiated according to the critical level of the object
\end{itemize}
    
- 그래서 이 논문에서는 다음 문제를 해결한다.
\begin{itemize}
    \item [Q1.] How to design the system architecture of RT-MOT that (a) not only provides a control knob to explore a tradeoff between timely execution and tracking accuracy, (b) but also offers a \jl{structure? interface?} to give preference to critical objects;
    and 
    \item [Q2.] How to efficiently utilize the proposed system architecture so as to maximize tracking accuracy for critical object (as well overall accuracy) while guaranteeing timely execution of every tracking.
    %tracking accuracy (giving preference to critical objects) while guaranteeing timely execution of every tracking.
\end{itemize}

- Q1의 해결을 위해 다음과 같은 RT-MOT system architecture를 제안한다.
\begin{itemize}
    \item detection과 association 부분에서 computation을 조절할 수 있도록 control interface 제공 (how에 관한 detail 여기에 서술) 
    \item prediction과  \jl{???} 부분에서 critical object에 대해 더 많은 resource를 할당할 수 있도록 control interface 제공하고 criticality 정보 제공 (how에 관한 detail 여기에 서술) \hbcmt{OK}
    \item 이러한 system architecture는 \jl{???} 측면에서 overhead를 줄여 Q2에서 효과적으로 (a)와 (b)를 달성 가능하게 하는 interface를 제공하는 역할을 함. \hbcmt{OK}
\end{itemize}

- Q2의 해결을 위해 다음과 같이 어떻게 detection과 association의 computation을 조절할지 정하는 scheduling framework을 제안한다.
\begin{itemize}
    \item O2 해결을 위해 기본적으로 detection과 association의 minimum computation을 기반으로 timing guarantees를 offline에서 달성함. online에서는 minimum computation의 deadline miss없이 실행할 수 있는 slack을 계산하여, 
    slack 내에서 minimum 이상의 computation을 함으로써 timing guarantee를 달성한다.
    %이를 minimum 이상의 computation을 task 별로 (inter-task) 그리고 각 task의 detection 및 association 간에 (intra-task) 어떻게 분배할지 결정한다. 따라서 이 framework 하에서 timing guarantee는 달성된다.
    \item accuracy를 향상하기 위해서는 slack을 효율적으로 
    (i) 같은 task 내에서 detection과 association 간에 (inter-task) 잘 나눠야 하며,
    (ii) 다른 task 간에 (inter-task) 잘 나눠야 하며, 
    (iii) 이 모든 것들이 object의 criticality를 반영하며,
    (iv) \jl{GPU call overhead?}를 고려해야 한다.
    \item 이를 위해 \jlcmt{여기에 우리의 scheduling policy 개발을 위해 motivational experiment를 통한 observation을 이야기 하고, 그것을 바탕으로 nice한 policy를 개발했다고 설명}
\end{itemize}

% \begin{itemize}
%     \item (백교수 아래 설명 참고) MOT 배경 설명, DNN-based MOT의 기본적인 구조 설명(detention, association, update, prediction).
%     \item (백교수 아래 설명 참고) 현재 MOT 들은 주로 high accuracy and average FPS를 주로 목적으로 하고 있어 safety-critical real-time systems에 적합하지 않음.
%     우리는 limited resource하에서 (i) timely execution of tracking should be guaranteed, (ii) tracking accuracy should be high, but differentiated according to the critical level of the object를 달성하는 것이 필요함.
%     \item 그래서 다음 문제를 해결한다.
%     (Q1) How to design the system architecture of RT-MOT that (a) not only provides a control knob to explore a tradeoff between timely execution and tracking accuracy, (b) but also offers a \jl{structure?} to give preference to critical objects;
%     and 
%     (Q2) How to efficiently utilize the proposed system architecture so as to maximize tracking accuracy (giving preference to critical objects) while guaranteeing timely execution of every tracking.
%     % \item (백교수 아래 설명 참고) 현재 MOT 연구 상황, safety-critical real-time systems에서의 새로운 MOT requirements: (i) timely execution of tracking should be guaranteed, (ii) tracking accuracy should be high, but differentiated according to the critical level of the object.
%     % \item DNN-based MOT의 기본적인 구조 설명: detection, association, update, prediction으로 나뉘어짐.
%     % \item 새로운 MOT requirement 달성에 어려운 점은?:
%     % (a) detection, association, update, prediction 으로 나누어져 있는 복잡한 MOT의 step들에서 (i)와 (ii)를 support할 수 있도록 하는 system architecture가 필요하
% \end{itemize}



-------------

\hbcmt{brief MOT introduction}
\begin{itemize}
	\item  MOT 는 객체의 과거, 현재, 미래의 경로예측까지 가능하게 하는 기술로 현대의 자율주행 시스템(또는 스마트 CCTV 등)에 널리 사용된다. 
	\item 자율주행에 MOT를 적용한 application로서 이러저러한 example들(보행자, 차량의 경로예측)이 있다.	
\end{itemize}	
~\\
\hbcmt{necessity of effective real-time scheduling for mixed-critical multi-object tracking (MC-MOT). detail한 기술 설명은 다음 paragraph에서}
\begin{itemize}
	\item  이러한 자율주행 시스템은 일반적으로 resource가 한정적인 특성이 있으며, real-time guarantee를 해주어야 한다는 requirement가 있다.
	\item  resource가 한정적이므로, requirement에 따라 선별적으로 resource를 allocation 해야 한다. 
	\item \textbf{우리의 주장은 critical(urgent)한 object과 그렇지 않은 object들이 존재하고, crtical한 object들을 한정적인 resource를 이용하여 우선적으로(이들의 accuracy를 최우선적으로) tracking하여야 한다는 것.}
	\item 예를 들어 ----- (a specific example here): 차와 사람의 속도를 파악하여, 나와의 충돌을 예상할 수 있는데, 일부는 critical하고 등등 
	%\item 선별적 resource allocation을 위해 critical 한 object에 우선적으로 computing power를 주어 tracking 하여야 한다. (while providing timing guarantee). $\leftarrow$좀 더 잘 쓰기.
	%\item 그리고, critical 하지 않은 object들을 위해서는 timing guarantee를 해치지 않는 선에서 남는 resource 를 allocation해야 한다.  
	\item critical한 object들은 수시로 그 대상자체가 변하며, 각각 다른 경로를 가지며 이동한다. 이를 한정적인 자원으로 지속적으로 tracking하는 것은 매우 challenging한 mission이다.
	\item 또한, critical한 object들을 tracking하는데 집중하며, 남은 computing power로 다른 object들도 효율적(즉, accuracy maximizing for non-critical objects)으로 tracking하여야 한다.
	\item \hb{Critical Object의 정의를 확실하게 언급할 것}
	%\item 이러한  scheduling framework를 구축하는 와중에 (기존 MOT 대비) accuracy loss를 최소화하고 computational overhead도 최소화 되어야 한다.  $\leftarrow$ 좀 애매함, 좀 더 잘 쓰기.
	%	\item State-of-the-art MOT는 accuracy 를 높이기 위해서 점점 DNN 을 사용하고, 이에 따라, 점점 요구되는 computation 이 heavy 해 지고 있다. 
	%	\item 따라서, MOT의 DNN execution 의 mandatory 한 부분과 optional 한 부분을 상황에 맞게 computing 하여 real-time guarantee (while minimizing accuracy loss)를 해주어야 한다.   = Goal	
\end{itemize}

~\\

\hbcmt{description of a state-of-the-art MOT technique}
\begin{itemize}
	\item MOT 중 tracking-by-detection은 각 frame의 detection의 결과를 이용하여(각 frame의 object들을 association) tracking하는 방법으로 이러저러한 장점으로 인해 가장 널리 사용되고 있는 방법 중 하나이다. 
	\item \hbcmt{tracking-by-detection의 기본적인 동작(concept)을 이해하기 위해 그림이 필요하다고 생각됨.}
	\item state-of-the-art tracking-by-detection MOT technique들은 정확도의 향상을 위해 DNN을 사용한다. 
	\item DNN based approach는 다음과 같은 4step으로 동작하는데: 1. detection (e.g., YOLOv5, Faster R-CNN), 2. association (e.g., OSnet-based feature extraction (cosine distance)+(마할라노비스 distance)), 3. update (e.g., 헝가리안 ID allocation) 4. prediction (e.g., 칼만필터) 
	\item DNN은 이 중 1. detection에서 object들의 localization과 classification을 위해 사용되며, 2. association에서 앞 뒤 frame에 존재하는 object들의 matching(feature를 뽑아서 유사도를 비교, 전통적인 위치기반 비교법에 비해 비약적인 accuracy상승을 보임)을 위해 사용된다. 
	\item 이 작업이 DNN-based MOT에서 computation load의 대부분을 차지한다 (up to 90\% in our experiment setting). 
	\item \textbf{자율주행 시스템의 fundamental constraint(limited resource) and requirement(timing guarantee, computation for mixed-critical objects?-좀더 잘쓰기)에도 불구하고 state-of-the-art MOT 기법은 accuracy 향상에만 치중하고 있으며, 특히 real-time guarantee와 mixed-critical object들을 동시에 고려한 선별적 tracking 기법(=scheduling platform)은 사실상 전무하다.}
\end{itemize}


~\\

\hbcmt{Problem definition}
\hb{우리는 문제를 이렇게 정의 할 수 있다. }
\begin{itemize}
	\item [Q.1] input image에서 어떻게 (pre-defined 된 정의를 따르는) critical한 object들을 효율적인 computation으로 찾아 낼 수 있나?
	\item [Q.2] 어떻게 Detection과 association에서 computation을 조절할 수 있나? (동시에 crtical object에 대한 accuracy 우선으로) accuracy vs fps tradeoff
	\item [Q.3] Q.2에 따른 platform에서 어떻게 MOT specific한 property를 이용하여 효율적으로(accuracy effective하게+schedulability guarnatee) 스케줄링 할 수 있나?
	
\end{itemize}

~\\
\hbcmt{our approach in overall}\hbcmt{현재 너무 디테일한데, high-level로 잘 쓸것} \hbcmt{DeepSORT를 modify한 approach라고 이야기 할 필요 전혀 없음!}
\begin{itemize}
	\item We propose MC-MOT(DNN-based real-time mixed-critical multi-object tracking and scheduling framework) that 서로 다른 critical를 가지는 object들를 추척하기 위해 DNN workload of detection, DNN workload of association을 dynamic하게 조절하고 scheduling 하는 framework를 제안한다.
	%\st{Under scheduling policy of MC-MOT, high-critical object들의 accuracy는 maximize하기 위해 resource가 우선적으로 allocate되며, remaining resource를 통해 low-critical object들을 위해 사용된다 while guaranteeing timely execution.}     
	%	\item MC-MOT consists of three components: MC-YOLO(1. detection), MC-AU(2. association\& 3. update), MC-Prediction(4. prediction) that are scheduled by global scheduler 
	
	%한정된 자원하에서 서로 다른 criticality를 가지는 object들을 고려하여 선별적으로 tracking하고 이를 위해 computing resource를 선별적으로 allocate(scheduling) 하는 while guaranteeing  timely execution = schedulability.
	\hbcmt{일단 scheduling 이야기는 나중에 추가시키자. idea brain storming 후에...}
	\item \hb{For Q2 at 1. Detection}, we propose MC-YOLO (mixed-critical objects detection and scheduling framework from YOLOv5) that is extended from YOLOv5.  
	%	\item 
	\item MC-YOLO는 먼저 input image의 high-critical한 object들이 존재할만한 영역과 그렇지 않은 영역을 분리하고, policy(depending on sub-scheduler)에 맞게 resize한 후 각각 DNN network(darknet)을 통과 시킨 후, 이 둘을 NMS로 합친다.
	\item \hb{For Q1 at 1. Detection}, 그 후, euclidean distance(and 마할라노비스 distance)를 이용하여\hbcmt{좀더 detail하게, 이해 되게 설명}, critical object들과 그렇지 않은 object들을 추출해 낸다. \hbcmt{DNN-SAM과 유사한 부분을 어떻게 defense할지?}
	%\item For 2. association: we propose MC-AS(mixed-critical objects-aware association(\&update) and scheduling framework(?))\hbcmt{새로운 이름이 필요할지?} that 제한된 computing resource하에서 criticality를 고려해 matching을 하고 computing load를 scheduling하는 framework.
	%\item MC-AS 역시 주어진(from parent scheduler) budget하에서 동작하는데, 먼저 sub-schduler가 for critical objects, for non-critical objects들을 위해 computing resource을 allocation한다. 
	\item \hb{For Q2 at 2.\&3. association(and update)}, we propose selective feature extraction and matching cascade scheduler에 의해 정해진 budget에 따라 선별적으로 object들의 feature 를 뽑는다.  
	\item 이 후, 선별적으로 association을 진행한다. feature가 뽑힌 objects들을 우선적(cosine distance+Mahalanobis distance)으로 매칭하고, 나머지 들은 \hbcmt{너무 detail한가?} IOU distance를 이용하여 matching 한다. 이 와중에 ID가 자동으로 할당 된다.
	%\item For 3. update(ID allocation)는 사실 2와 같이 이루어짐
	\item \hb{For Q1 at 4. prediction} 은 detect된 object들이 어디에 있을지 예상하고(from 칼만필터), 모든 object들의 time-to-collosion을 구한다. 
	\item 이를 기반으로 다음 frame에서 critical object들이 존재할 수 있는 region을 proposal한다.  
	\item \hb{For Q3}, 스케줄링은 MOT specific한 이러저러한 것을 이용해서 동작한다. GPU call 줄이려고 노력했고, MOT의 특성인 history를 이용했다. 이용한 것과 안한것의 성능차이가 매우 많이 난다. 
	\item schedulability analysis도 제안
\end{itemize}


~\\	


\hbcmt{Advantages of our approach}\hb{논의필요}
\begin{itemize}
	\item  DNN-based MOT를 함에 있어서, dynamic하게 변하는 object들의 criticality를 지속적으로 tracking(update)하고 이를 위해 선별적으로 scheduling(for timing guarantee)한다.  
	\item  
	\item 
	\item 해당 approach는 카메라만(다른 sensor 필요없이)을 이용하여 region proposal and tracking different critical objects
\end{itemize}

\hbcmt{강조 할 부분}\hb{작성중}
\begin{itemize}
	\item  (first 라고 주장 할 수 있나?), To the best of our knowledge, it first "provides timing guarantee for SOTA DNN-based MOT" 
	\item  
\end{itemize}


\hbcmt{contributions}\hb{작성중}
\begin{itemize}
	\item  
	\item  
	\item 
	\item 
\end{itemize}

~\\


==> old_05scheduling.tex <==
%\section{scheduling and schedulability}
\section{Scheduling Framework}
\label{sec:scheduling}

\hbcmt{section intro}
\begin{itemize}
	\item \hb{Q2를 위해 O3, O4, O5, O6을 이용.}
	\item 이를 위해 먼저 MC-MOT의 scheduling framework를 위한 task model을 만든다.  
	\item O3, O4, O5를 이용해서 먼저 naive version을 만들고
	\item (O3, O4, O5) + O6를 이용해서 slack version을 만든다. 
\end{itemize}


\subsection{Task model}

According to the system design in Section~\ref{sec:system_design},
each task periodically performs MOT for a series of input images from a camera.
%detection, association, update and prediction for an input image from a camera.
We represent each task as a periodic task model~\cite{LiLa73} as follows.
A task $\tau_i\in\tau$ is specified by $(\tau_i^{D}, \tau_i^{A}, T_i)$,
where $\tau_i^{D}$ is a sub-task of $\tau_i$ for detection,
$\tau_i^A$ is a sub-task of $\tau_i$ for association, update and prediction,
and $T_i$ is the period of $\tau_i$. 
A task $\tau_i\in\tau$ invokes a series of jobs periodically.
A job of $\tau_i$, once released at $t_0$, should finish the execution of its sub-job of $\tau_i^D$ 
and then that of $\tau_i^A$ (sequentially) until $t_0+T_i$;
the time difference between the release time of a job of $\tau_i$ and the next job of $\tau_i$ 
is exactly $T_i$.
%the separation of the release time of a job of $\tau_i$ and the next job of $\tau_i$ 
%is exactly $T_i$.


% Under MC-MOT, 하나의 카메라는 주기적으로 input image를 받아들이고 각 input image에 대해 MOT 의 4steps(1. detection (via MC-YOLO), 2.\&3. association and update, 4. prediction)를 수행한다.  
% 이러한 하나의 카메라를 a periodic task $\tau_i$로 표현하며, $n$개의 $\tau_i$ 는 $\tau_i \in \tau$를 만족한다. 
% A task $\tau_i$ consists of two subtasks $\tau_i^{D}$ representing 1. detection (via MC-YOLO) and $\tau_i^{A}$ representing the other steps 2.\&3.\&4. association, update, and prediction.
% Then, two subtasks share the same deadline $T_i$ and $D_i$, which is specified by $\tau_i = (\tau_i^{D}, \tau_i^{A}, D_i, T_i)$. 
% That is, each job of $\tau_i^{D}$ and $\tau_i^{A}$ is generated infinitely and its execution should be complete within $D_i$ after its generation(release).  

\jlcmt{이 문단 추후에 수정: 방법이 바뀌어서, ROI는 min부터 max인가? 아니면 ROI도 skip하고 뒤에 location of previous objects만 하는게 min인가?
min일때는 ROI를 최소 크기로 돌린다(256). ROI 외에 region 은 뒤에서 커버한다. (무조건 full size이므로 뒤에 단계는 WCET가 바뀌지 않는다.
min과 max 사이의 ROI는 어떻게 해야 하나? (앞에서 서술하고 뒤에서는 option 만 나열)} 

A sub-task $\tau_i^{D}$ is presented by $\tau_i^{D} = (R_i, C_i^{D}(s_i))$ where $R_i = \{(x,y), (w,h)\}$ is specified by the center position $(x,y)$ and the maximum (resized) image size $(w=256,h=x)$ of RoI, and $C_i^{D}(s_i)$ is the $\tau_i^{D}$'s worst-case execution time that can vary according to the resized total image $s_i \in S_i = \{0, 160, 256, 320,$ $416, 512, 608, 672 \}$.
Note $s_i$ indicates height of the resized total image, and then width is determined by $s_i * xx$.
That is, as MC-YOLO conducts inferences twice (once with the fixed (resized) size $(w=256,h=x)$ of RoI, then with the resized total image), the worst-case inference time for RoI is fixed, while that for the resized total image is determined by $s_i$.  
Thus, we let $c_i^{infer}(s_i)$ be the total inference time for MC-YOLO that has the eight different worst-case execution times; minimum and maximum are $c_i^{infer}(0)$ and $c_i^{infer}(672,x)$. 
Then, $C_i^{D}(s_i)$ is obtained by the following:



\begin{align}
	C_i^{D}(s_i) = c^{pre} + c_i^{infer}(s_i) + c^{nms} + c^{select}
\end{align}

\noindent
where $c^{pre}$, $c^{nms}$, and $c^{select}$ denote the worst-case execution times for RoI를 이전 fame의 $\tau_i^{A}$으로부터 받아서 image를 crop하고 (critical, non-critical images 모두) resize하는 module (즉, preprocessing 과정), NMS module, and critical한 object들을 선별하는 module.

\jlcmt{이 문단 추후에 수정}  A sub-task $\tau_i^{A}$ is specified by $\tau_i^{A} = (O_i, C_i^{A}(f_i))$ where $O_i$는 현재 시간 t에서 $\tau_i^{D}$ 로부터 추출 된 object들, $f_i$는 $O_i$ 중 feature extractoin과 matching cascade대상이 되는 object들의 최대 개수이다. 
Note that $O_i$는 $\tau_i^{D}$이 실행을 마쳐야 결정된다. 
따라서 $f_i$는 $\tau_i^{D}$의 실행전에 결정되는 설정치이며, $\tau_i^{D}$의 실행 후에 $f_i \le |O_i|$를 만족하면 $O_i$의 모든 object가 (selective feature extraction module)+(selective matching cascade module)의 대상이 되며, 
$f_i > |O_i|$ 이면 $O_i$ 중 $f_i$개수만 대상이 된다. 
critical object들이 먼저 $f_i$에 포함되며(critical object들 간 순서는 없음), critical object의 개수가 $f_i$보다 많을 시 non-critical object가 순서(randomly) 없이 포함된다.  
%$O^{f}_i \subset O_i$ 는 $O_i$ 중 feature extraction의 대상이 되는 object들.  
$c_i^{feature}(f_i)$는 the worst-case execution time of (selective feature extraction module)+(selective matching cascade module)로써, $f_i$ 에 따라 서로 다른 8가지의 wort-case execution을 가지는데, (그 구간은 ${0, 0-4, 5-9, 10-14, 15-19, 20-24, 25-29, 30-34}$) $f_i \in F_i = \{0, 4, 9, 14, 19, 24, 29, 34\}$ 이다(0일때 $c_i^{feature}(f_i)$가 zero라는 뜻, 우리는 object개수가 34가 넘지 않는다고 가정한다). 
참고로 $f_i$는 scheduling policy에 따라 0 부터 34 까지 변할 수 있으며, critical object들부터 채워진다. 
즉, $C_i^{A}(f_i)$는 $f_i$에 따라 서로 다른 8개의 worst-case execution time을 가지는데, 다음과 같이 구해 진다.  

\begin{align}
C_i^{A}(f_i) = &c_i^{feature}(f_i) + c_i^{IoU} + c_i^{kalman} \nonumber\\
						&+ c_i^{critical} + c_i^{RoI}
\end{align}

\noindent
where, $c_i^{IoU}$, $c_i^{kalman}$, $c_i^{critical}$, and $c_i^{RoI}$ are IoU matching module, 칼만필터 update, 
time-to-collision 계산(+criticality(for objects) update), and RoI proposal.  

\jlcmt{이 문단 추후에 수정} Each subtask is executed non-preemptively, which implies that a higher priority job cannot preempt any currently executing job of a subtask.
However, a subtask can execute between $\tau_i^{D}$ and $\tau_i^{A}$ of the same task $\tau_i$.
$s_i$ and $f_i$ are determined online, but the eight different worst-case execution times of $c_i^{infer}(s_i)$ and $c_i^{feature}(f_i)$ are predetermined(by measured) offline.
We assume that each job of $\tau_i^{D}$ and $\tau_i^{A}$ is released at the same time periodically, 
but $s_i$ and $f_i$ can be determined any time before the job of $\tau_i^{D}$ or $\tau_i^{A}$ begins its execution, according to the considered scheduling algorithm.
%For ease of presentation, we let $C_i^{D}(0)=C_i^{D}(min)$ and $C_i^{A}(0)=C_i^{A}(min)$ indicating that MC-MOT가 critical object를 잘 탐지해내고 추적하기 위해   $\tau_i^D$ 과 $\tau_i^A$에서 필요한 최소한의 worst-case execution time. 

\jlcmt{active job (sub-job)의 정의}

% \begin{figure*}[t!]
% 	\centering 
% 	\includegraphics[width=0.9\linewidth]{figures/scheduling.pdf}
	
% 	\caption{scheduling}
% 	\label{fig:scheduling}
% \end{figure*}

\subsection{Underlying ideas of proposed algorithms}


\jlcmt{4.26 백교수와의 회의 내용:

FP 적용 (RM이 Optimal인지 확인 필요)

L. George, N. Rivierre, and M. Spuri, “Preemptive and non-preemptive
real-time uniprocessor scheduling,” Ph.D. dissertation, Inria, 1996 \cite{GRS96} 논문의 Theorem 15를 offline analysis로 사용

Run-time: execution을 더 하여도 priority가 낮은 task (interference)와 높은 task (blocking) 관점에서 scheduling이 가능한지에 대한 table을 offline에 만들어놓고, 이것을 이용하여 run-time에 schedulability를 compromise하지 않고 실행가능한지 체크하여, 가능한 max execution time을 계산한다.

계산한 max execution time 중 얼만큼 실행할지는 정하는것이 필요하다. 

}

-\\-\\-\\-\\-\\

\begin{lemma} [From \cite{GRS96} \jlcmt{42p, Def. 3}]
    A level-i busy period is defined as a processor busy period in which only instances of tasks with priority higher than or equal to that of $\tau_i$ execute.
    The length of the longest level-i busy period under non-preemptive FP, denoted by $L_i$,
    is calculated as follows.
    
    \jlcmt{원래 식}
    \small
    \begin{align}
        L_i = \max_{\tau_j\in\textsf{LP}(\tau_i)} (C_j-1) + \sum_{\tau_h\in\textsf{HP}(\tau_i)\cup\{\tau_i\}} \bigg\lceil\frac{L_i}{T_h} \bigg\rceil\cdot C_h.
    \end{align}
    \normalsize
    
    \jlcmt{converge 할때까지 계산 필요, quantum을 1로 하는게 아니면 -1 삭제 필요}
    
    \jlcmt{우리 system model}
    \small
    \begin{align}
        L_i = \max_{\tau_j\in\textsf{LP}(\tau_i)} \max(C_j^D(0)-1, C_j^A(0)-1) + \nonumber\\ \sum_{\tau_h\in\textsf{HP}(\tau_i)\cup\{\tau_i\}} \bigg\lceil\frac{L_i}{T_h} \bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big).
    \end{align}
    \normalsize
\end{lemma}

-\\

\begin{lemma} [From \cite{GRS96} \jlcmt{29p, Thm. 15}]
    The worst-case response time of $\tau_i$ under non-preemptive FP is calculated by 
    
    \jlcmt{원래 식}
    \small
    \begin{align}
        R_i = \max_{q=0, 1, ..., Q} (w_{i,q} + C_i-q\cdot T_i),
    \end{align}
    \normalsize
    
    \noindent where 
    \small
    \begin{align}
        w_{i,q} = q\cdot C_i + \sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg(1+\bigg\lfloor\frac{w_{i,q}}{T_h} \bigg\rfloor\bigg)\cdot C_h + \max_{\tau_j\in\textsf{LP}(\tau_i)} (C_j-1)
    \end{align}
    \normalsize
    and $Q=\lfloor L_i/T_i\rfloor$.
    
    \jlcmt{converge 할때까지 계산 필요, quantum을 1로 하는게 아니면 -1 삭제 필요}
    
    \jlcmt{우리 system model}
    \small
    \begin{align}
        R_i = \max_{q=0, 1, ..., Q} \big(w_{i,q} + C_i^D(0)+C_i^A(0)-q\cdot T_i\big),
    \end{align}
    \normalsize
    
    \noindent where 
    \small
    \begin{align}
        w_{i,q} = q\cdot \big(C_i^D(0)+C_i^A(0)\big) + \nonumber\\
        \sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg(1+\bigg\lfloor\frac{w_{i,q}}{T_h} \bigg\rfloor\bigg)\cdot \big(C_h^D(0)+C_h^A(0)\big) + \nonumber\\
        \max_{\tau_j\in\textsf{LP}(\tau_i)} \max(C_j^D(0)-1, C_j^A(0)-1)
    \end{align}
    \normalsize
    and $Q=\lfloor L_i/T_i\rfloor$.
\end{lemma}

-\\

Run-time에는 실행을 시작하려고 하는 $\tau_k$의 execution을 $C_i^D(0)$과 $C_i^A(0)$ 보다 크게 하려고 할때 $\tau_h\in\textsf{HP}(\tau_k)$와 $\tau_j\in\textsf{LP}(\tau_k)$에 속하는 task들이 schedulable 한지 확인해야 한다.

1. $\tau_h\in\textsf{HP}(\tau_k)$에 대해서:


각 $\tau_h$ 들에 대해 앞서 Lemma 두개에서 $\tau_k$의 $C_k^D$ 또는 $C_k^A$가 어디까지 늘어나도  $\tau_h$가 schedulable 한지 미리 offline으로 구해 놓는다. 이를 $B_{h\leftarrow k}^\testsf{MAX}$라고 하자. 
현재  $\tau_k$가 실행하려고 한다는 뜻은 그보다 높은 priority는 active job이 없다는 뜻이다.
따라서 $\tau_k$가 실행을 시작 하려고 하는 현재 시점을 $t_0$ 라고 하고, $\tau_h$의 다음 가장 빠른 release 시점을 $t_h$ ($>t_0$)라고 하면, $C_k^D$와 $C_k^A$는 $B_{h\leftarrow k}^\testsf{MAX}+(t_h-t_0)$까지 늘어나도 $\tau_h$의 schedulability를 compromise 하지 않는다. \jlcmt{여기서 DNN-SAM은 strictly periodic 이었는데, 우리는 sporadic도 커버 할듯}

2. $\tau_j\in\textsf{LP}(\tau_k)$에 대해서:

1번의 $\tau_h$과는 다르게 $\tau_j$는 $\tau_k$가 실행을 시작하려고 하는 현재 시점 $t_0$에 active job일 수 있다. 


3. $\tau_k$ 본인에 대해서:


-\\


%\jlcmt{위의 내용은 arbitrary deadline에 관한 것이고, constrained-deadline이나 T=D 의 경우 ``Non-preemptive Fixed priority scheduling of hard real-time periodic tasks'' 논문의 Theorem 1을 쓰면 된다.   }

\jlcmt{위의 내용은 arbitrary deadline에 관한 것이고, constrained-deadline이나 T=D 의 경우는 ``Effective Analysis for Engineering Real-Time Fixed Priority Schedulers'' 
논문의 (1)식을 활용하면 된다. }


(preemptive 식에 non-preemptive blocking만 고려)
    \small
    \begin{align}
        R_i = C_i^D+C_i^A+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{R_i}{T_h}\bigg\rceil\cdot (C_h^D+C_h^A)
    \end{align}
    \normalsize
    
    
    
    %     \small
    % \begin{align}
    %     R_i' = C_i^D+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{R_i'}{T_h}\bigg\rceil\cdot C_h
    % \end{align}
    % \normalsize

-\\

($C_i^A$ 부분이 시작하는 시점($R_i'$)만 구하면 response time을 구할 수 있다는 성질 이용)
    \small
    \begin{align}
        R_i' = C_i^D+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg(1+\bigg\lfloor\frac{R_i'}{T_h}\bigg\rfloor\bigg)\cdot (C_h^D+C_h^A)
    \end{align}
    \normalsize
    
    $R_i=R_i'+C_i^A$

-\\

RTA 대신 간단한 DA를 적용하고자 한다면

\small
    \begin{align}
        C_i^D+C_i^A+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{T_i}{T_h}\bigg\rceil\cdot (C_h^D+C_h^A) \le T_i
    \end{align}
    \normalsize


-\\

-----------------------

$***$ Offline analysis

    \small
    \begin{align}
        C_i^D(0)+C_i^A(0)+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{T_i}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \le T_i
    \end{align}
    \normalsize

위의 식에서 RHS-LHS를 $M_i$이라고 하자.
그러면 $\tau_i$는 Blocking을 $B_i+M_i$까지 받거나, 추가적인 interference를 $M_i$ 만큼 받아도 schedulable 하다.

-\\

$***$ Online analysis

-\\

$\bullet$ Case-D: $\tau_i^D$가 $t$에 실행을 시작할때 $\tau_i^D$의 실행 시간이 $C_i^D$를 뛰어넘어 얼마만큼 길어져도 되는지 살펴보자. 

-\\

$\bullet$ Case-D1: $\tau_i^D$의 실행이 $\tau_h\in\textsf{HP}(\tau_i)$의 schedulability에 미치는 영향 계산.

$t$초에 $\tau_i^D$가 실행을 시작한다는 뜻은 $t$초에 active한 $\tau_h$가 존재하지 않는다는 의미임.
$t$초 이후에 가장 빠른 $\tau_h$의 job release time을 $r_h(t)$라고 하자.
그리고, $t$초 이후에 가장 빠른 $\tau_i$의 job release time (= 현재 $\tau_i$'s job의 deadline)을 $r_i(t)$라고 하자. $r_h(t)< r_i(t)$인 모든 $\tau_h$에 대해서 아래의 식을 만족해야 한다.

%$r_h(t)-t$ 보다 $C_i^D$가 작은 경우: 아무런 영향이 없음. (아래 식을 만족 안하면 $C_i^D\le r_h(t)-t$가 최종 식)

%$r_h(t)-t$ 보다 $C_i^D$가 큰 경우: 아래의 식을 만족해야 함.

    \small
    \begin{align}
        C_i^D+ \nonumber\\ \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | r_{h2}(t)<r_h(t)+T_h} \bigg\lceil\frac{r_h(t)+T_h-r_{h2}(t)}{T_{h2}}\bigg\rceil \nonumber\\\cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le T_h+\big(r_h(t)-t\bit)
    \end{align}
    \normalsize
    
    %     \small
    % \begin{align}
    %     C_i^D-\big(r_h(t)-t\big)+ \nonumber\\ \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | r_{h2}(t)<r_h(t)+T_h} \bigg\lceil\frac{r_h(t)+T_h-r_{h2}(t)}{T_{h2}}\bigg\rceil \nonumber\\\cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
    %     \le T_h
    % \end{align}
    % \normalsize


    % \small
    % \begin{align}
    %     C_i^D\le r_h(t)-t+B_h+M_h
    % \end{align}
    % \normalsize


%$C_i^D\le r_h(t)+B_h+M_h-t$ 가 성립해야 한다.

-\\

$\bullet$ Case-D2: $\tau_i^D$의 실행이 $\tau_i^D$와 $\tau_i^A$의 schedulaiblity에 미치는 영향 계산.

$t$초에 $\tau_i^D$가 실행을 시작한다는 뜻은 $t$초에 active한 $\tau_h$가 존재하지 않는다는 의미임.
$t$초 이후에 가장 빠른 $\tau_h$의 job release time을 $r_h(t)$라고 하자.
그리고, $t$초 이후에 가장 빠른 $\tau_i$의 job release time (= 현재 $\tau_i$'s job의 deadline)을 $r_i(t)$라고 하자.
그러면 offline analysis 식은 아래와 같이 바뀐다. (이 경우 blocking은 없음)

    \small
    \begin{align}
        C_i^D+C_i^A(0)+ \nonumber\\ \sum_{\tau_h\in\textsf{HP}(\tau_i) | r_h(t)<r_i(t)} \bigg\lceil\frac{r_i(t)-r_h(t)}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \nonumber\\
        \le r_i(t)-t
    \end{align}
    \normalsize




-\\

$\bullet$ Case-D3: $\tau_i^D$의 실행이 $\tau_j\in\textsf{LP}(\tau_i)$의 schedulability에 미치는 영향 계산.

1) $t$초에 active한 $\tau_j$의 job의 경우:

$t$초 이후에 가장 빠른 $\tau_h$의 job release time을 $r_h(t)$라고 하자.
그리고, $t$초 이후에 가장 빠른 $\tau_i$의 job release time (= 현재 $\tau_i$'s job의 deadline)을 $r_i(t)$라고 하자.
$t$초 이후에 가장 빠른 $\tau_j$의 job release time (= 현재 $\tau_j$'s job의 deadline)을 $r_j(t)$라고 하자.

$\tau_j$의 schedulability는 다음과 같이 구할 수 있다.

-\\

1-1) $\tau_j$의 $\tau_j^D$가 $t$전에 아직 실행되지 않은 경우:

% -\\

% 1-1-1) $r_j(t)\le r_i(t)$ 인 경우:

    \small
    \begin{align}
        C_j^D(0)+C_j^A(0)+ C_i^D+C_i^A(0) + \nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | t\le r_{h2}(t)<r_j(t)} \bigg\lceil\frac{r_j(t)-r_{h2}(t)}{T_{h2}}\bigg\rceil\cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le r_j(t)-t
    \end{align}
    \normalsize
    
    \jlcmt{위의 식에서  $\tau_{h2}$ 인데 $\tau_i$보다 priority가 낮은 작업은 $t$초 이전에 release 하고 끝나지 않는 job이 있을수 있음. 이경우는 따로 더해줘야 함. 해당 job의 $\tau_{h2}^D$가 실행되지 않았으면 $C_{h2}^D(0)+C_{h2}^A(0)$를 더해야 하고, 해당 job의 $\tau_{h2}^D$는 실행되고 $\tau_{h2}^A$만 실행되지 않았으면 $C_{h2}^A(0)$만 더해 주면 됨. }

% 1-1-2) $r_j(t) > r_i(t)$ 인 경우:

% 위의 식에서 $\min( , r_j(t)-t)$ 만 제외하면 됨.

-\\

1-2) $\tau_j$의 $\tau_j^D$가 $t$전에 실행되고 $\tau_j^A$가 $t$전에 아직 실행되지 않은 경우:

-\\

% 1-2-1) $r_j(t)\le r_i(t)$ 인 경우:

위의 식에서 $C_j^D(0)$ 만 삭제하면 됨.

% 1-1-1) 식에서 $C_j^D(0)$ 만 삭제하면 됨.

% 1-2-2) $r_j(t) > r_i(t)$ 인 경우:

% 1-1-2) 식에서 $C_j^D(0)$ 만 삭제하면 됨.

-\\

2) $t$초 이후에 release 할 $\tau_j$의 job의 경우 (그리고 $r_j(t) < r_i(t)$를 만족하는 경우): 


    % \small
    % \begin{align}
    %     \min\big(r_i(t)-r_j(t), C_i^D+C_i^A(0)\big) + \nonumber \\
    %     %\max\Big(0, C_i^D+C_i^A(0)-\big(r_j(t)-t\big)\Big) + \nonumber\\ 
    %     \bigg\lceil\frac{\max\big(0,r_j(t)+T_j-r_i(t)\big)}{T_i}\bigg\rceil\cdot \big(C_i^D(0)+C_i^A(0)\big) \nonumber\\
    %     \le \bigg\lceil\frac{T_j}{T_i}\bigg\rceil\cdot \big(C_i^D(0)+C_i^A(0)\big) + B_h + M_h
    % \end{align}
    % \normalsize
    
    \small
    \begin{align}
        C_j^D(0)+C_j^A(0)+ C_i^D+C_i^A(0) + \nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | t\le r_{h2}(t)<r_j(t)+T_j} \bigg\lceil\frac{r_j(t)+T_j-r_{h2}(t)}{T_{h2}}\bigg\rceil\nonumber\\
        \cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le T_j+\big(r_j(t)-t\big)
    \end{align}
    \normalsize

    \jlcmt{위의 식에서  $\tau_{h2}$ 인데 $\tau_i$보다 priority가 낮은 작업은 $t$초 이전에 release 하고 끝나지 않는 job이 있을수 있음. 이경우는 따로 더해줘야 함. 해당 job의 $\tau_{h2}^D$가 실행되지 않았으면 $C_{h2}^D(0)+C_{h2}^A(0)$를 더해야 하고, 해당 job의 $\tau_{h2}^D$는 실행되고 $\tau_{h2}^A$만 실행되지 않았으면 $C_{h2}^A(0)$만 더해 주면 됨. }

-\\

Case-D1, Case-D2, Case-D3에서 나오는 모든 식들은 $C_i^D\le constant$의 형태이며, 모든 식을 AND 조건으로 하여 가장 tight한 식을 뽑아내면, 그것이 $C_i^D$의 최종 constraint이다. 

-\\

\jlcmt{Case-A는 Case-D에서 $C_i^D$를 $C_i^A$로 바꾸고, $C_i^A(0)$를 삭제하면 됨.}

% $\bullet$ Case-A: $\tau_i^A$가 $t$에 실행을 시작할때 $\tau_i^A$의 실행 시간이 $C_i^A$를 뛰어넘어 얼마만큼 길어져도 되는지 살펴보자. 

% -\\

% $\bullet$ Case-A1: $\tau_i^A$의 실행이 $\tau_h\in\textsf{HP}(\tau_i)$의 schedulability에 미치는 영향 계산.

% Case-D1과 동일함.

%     \small
%     \begin{align}
%         C_i^A\le r_h(t)+B_h+M_h-t
%     \end{align}
%     \normalsize

% -\\

% $\bullet$ Case-A2: $\tau_i^A$의 실행이 $\tau_i^A$의 schedulaiblity에 미치는 영향 계산.

% Case-D2와 동일한 방법.

% 그러면 offline analysis 식은 아래와 같이 바뀐다. (이 경우 blocking은 없음)

%     \small
%     \begin{align}
%         C_i^A+ \nonumber\\ \sum_{\tau_h\in\textsf{HP}(\tau_i) | r_h(t)<r_i(t)} \bigg\lceil\frac{r_i(t)-r_h(t)}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \nonumber\\
%         \le r_i(t)-t
%     \end{align}
%     \normalsize


% -\\

% $\bullet$ Case-A3: $\tau_i^A$의 실행이 $\tau_j\in\textsf{LP}(\tau_i)$의 schedulability에 미치는 영향 계산.

% 1) $t$초에 active한 $\tau_j$의 job의 경우:

% -\\

% 1-1) $\tau_j$의 $\tau_j^D$가 $t$전에 아직 실행되지 않은 경우:

%     \small
%     \begin{align}
%         C_j^D(0)+C_j^A(0)+ C_i^A + \nonumber\\ 
%         \sum_{\tau_h\in\textsf{HP}(\tau_j) | r_h(t)<r_j(t)} \bigg\lceil\frac{r_j(t)-r_h(t)}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \nonumber\\
%         \le r_j(t)-t
%     \end{align}
%     \normalsize

% -\\

% 1-2) $\tau_j$의 $\tau_j^D$가 $t$전에 실행되고 $\tau_j^A$가 $t$전에 아직 실행되지 않은 경우:

% 위의 식에서 $C_j^D(0)$ 만 삭제하면 됨.

% -\\

% 2) $t$초 이후에 release 할 $\tau_j$의 job의 경우 (즉, $r_j(t) < r_i(t)$): 


%     \small
%     \begin{align}
%         C_i^A-\big(r_j(t)-t)\big + \nonumber\\ \bigg\lceil\frac{\max\big(0,r_j(t)+T_j-r_i(t)\big)}{T_i}\bigg\rceil\cdot \big(C_i^D(0)+C_i^A(0)\big) \nonumber\\
%         \le \bigg\lceil\frac{T_j}{T_i}\bigg\rceil\cdot \big(C_i^D(0)+C_i^A(0)\big) + B_h + M_h
%     \end{align}
%     \normalsize

% -\\

% Case-A1, Case-A2, Case-A3에서 나오는 모든 식들은 $C_i^A\le constant$의 형태이며, 모든 식을 AND 조건으로 하여 가장 tight한 식을 뽑아내면, 그것이 $C_i^A$의 최종 constraint이다. 

% -\\

\newpage

--------------------------------------

$***$ Offline analysis \jlcmt{다시 서술: OLD}

    \small
    \begin{align}
        C_i^D(0)+C_i^A(0)+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{T_i}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \le T_i
    \end{align}
    \normalsize
    
    \small
    \begin{align}
        R_i = C_i^D(0)+C_i^A(0)+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{R_i}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\bit)
    \end{align}
    \normalsize
    
차례대로 DA, RTA임. 무엇을 적용해도 됨. 여기서 $B_i=\max_{\tau_j\in\textsf{LP}(\tau_i)} C_j$ (또는 quantum이 1로 주어져 있으면 $C_j-1$).

% 위의 식에서 RHS-LHS를 $M_i$이라고 하자.
% 그러면 $\tau_i$는 Blocking을 $B_i+M_i$까지 받거나, 추가적인 interference를 $M_i$ 만큼 받아도 schedulable 하다.

-\\

$***$ Online analysis \jlcmt{다시 서술: OLD}

-\\

Definition. $S_i(t)$는 $\tau_i$의 $t$초에서의 state를 의미함. $S_i(t)=\textsf{DT}$는 Detection과 Association을 실행해야 할 $\tau_i$의 job이 $t$초에 존재함을 의미함. $S_i(t)=\textsf{AS}$는 (Detection은 $t$초 이전에 이미 실행하였고) Association을 실행해야 할 $\tau_i$의 job이 $t$초에 존재함을 의미함. $S_i(t)=\textsf{NO}$는 실행이 남은 $\tau_i$의 job이 $t$초에 존재하지 않음을 의미함.

-\\

Definition. $t$초나 $t$초 이후에 가장 빠른 $\tau_i$의 job release time을 $r_i(t)$라고 하자.

-\\

$\bullet$ Case-D: $\tau_i^D$가 $t$에 실행을 시작할때 (즉, $S_i(t)=\textsf{DT}$) $\tau_i^D$의 실행 시간이 $C_i^D(0)$를 뛰어넘어 얼마만큼 길어져도 되는지 살펴보자. 

-\\

$\bullet$ Case-D1: $\tau_i^D$의 실행이 $\tau_h\in\textsf{HP}(\tau_i)$의 schedulability에 미치는 영향 계산.

$t$초에 $\tau_i^D$가 실행을 시작한다는 뜻은 모든 $S_h(t)$ 는 $\textsf{NO}$임. 

By definition, $r_i(t)$는 현재 $\tau_i$'s job의 deadline 이기도 하다. 
그러면 $r_h(t)<r_i(t)$ 인 모든 $\tau_h$에 대해서 아래의 식을 만족하면, 
$C_i^D$가 $C_i^D(0)$ 보다 커져도 $r_h(t)$에 release 하는 $\tau_h$의 job이 deadline miss 하지 않는다.

    \small
    \begin{align}
        C_i^D+ C_h^D(0)+C_h^A(0)+\nonumber\\ \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | r_{h2}(t)<r_h(t)+T_h} \bigg\lceil\frac{r_h(t)+T_h-r_{h2}(t)}{T_{h2}}\bigg\rceil \nonumber\\\cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le T_h+\big(r_h(t)-t\bit)
    \end{align}
    \normalsize

-\\

$\bullet$ Case-D2: $\tau_i^D$의 실행시간을 증가하는 것이 $\tau_i$ 자신의 schedulaiblity에 미치는 영향 계산.

$t$초에 $\tau_i^D$가 실행을 시작한다는 뜻은 모든 $S_h(t)$ 는 $\textsf{NO}$임.

그러면 offline analysis 식은 아래와 같이 바뀐다. (이 경우 blocking은 없음)

    \small
    \begin{align}
        C_i^D+C_i^A(0)+ \nonumber\\ \sum_{\tau_h\in\textsf{HP}(\tau_i) | r_h(t)<r_i(t)} \bigg\lceil\frac{r_i(t)-r_h(t)}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \nonumber\\
        \le r_i(t)-t
    \end{align}
    \normalsize

-\\

$\bullet$ Case-D3: $\tau_i^D$의 실행이 $\tau_j\in\textsf{LP}(\tau_i)$의 schedulability에 미치는 영향 계산.

$S_j(t)$ 가 $\textsf{DT}$, $\textsf{AS}$, $\textsf{NO}$ 인지에 따라 다르게 처리해야 하는데, 어쨋든 $\tau_j$의 job중 맨 앞에 있는 $\tau_j$의 job 하나만 고려하면 그 다음 $\tau_j$의 job 들은 고려할 필요가 없다.
그 이유는 맨 앞의 job이 schedulable 했다는 이야기는 이미 level-i busy interval이 끝나고 $\tau_j$의 실행이 되었다는 의미이므로 $C_i^D$가 커진 효과가 없다. (원래 $C_i^D(0)$ 기준 schedulability는 이미 offline에서 했으므로 OK)

1) $S_j(t)=\textsf{DT}$의 경우:

    \small
    \begin{align}
        C_j^D(0)+C_j^A(0)+ C_i^D+C_i^A(0) + \nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{DT}} \big(C_{h2}^D(0)+ C_{h2}^A(0)\big) +
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{AS}} C_{h2}^A(0) + \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | t < r_{h2}(t)<r_j(t)} \bigg\lceil\frac{r_j(t)-r_{h2}(t)}{T_{h2}}\bigg\rceil\cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le r_j(t)-t
    \end{align}
    \normalsize

-\\

2) $S_j(t)=\textsf{AS}$의 경우:

위의 식에서 $C_j^D(0)$ 만 삭제하면 됨.

-\\

3) $S_j(t)=\textsf{NO}$의 경우:


    \small
    \begin{align}
        C_j^D(0)+C_j^A(0)+ C_i^D+C_i^A(0) + \nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{DT}} \big(C_{h2}^D(0)+ C_{h2}^A(0)\big) +
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{AS}} C_{h2}^A(0) + \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | t < r_{h2}(t)<r_j(t)+T_j} \bigg\lceil\frac{r_j(t)+T_j-r_{h2}(t)}{T_{h2}}\bigg\rceil\nonumber\\
        \cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le T_j+\big(r_j(t)-t\big)
    \end{align}
    \normalsize

-\\

Case-D1, Case-D2, Case-D3에서 나오는 모든 식들은 $C_i^D\le constant$의 형태이며, 모든 식을 AND 조건으로 하여 가장 tight한 식을 뽑아내면, 그것이 $C_i^D$의 최종 constraint이다. 

-\\

$\bullet$ Case-A: $\tau_i^A$가 $t$에 실행을 시작할때 (즉, $S_i(t)=\textsf{AS}$) $\tau_i^A$의 실행 시간이 $C_i^A$를 뛰어넘어 얼마만큼 길어져도 되는지 살펴보자. 

\jlcmt{Case-A는 Case-D의 모든 subcase 식에서 $C_i^D$만 있는 경우는 $C_i^D$를 $C_i^A$로 바꾸고, $C_i^D+C_i^A(0)$가 있는 경우는 $C_i^D+C_i^A(0)$를 $C_i^A$로 바꾸면 됨.}

-\\-\\-\\-\\-\\

\newpage

-\\

\newpage

--------------------------------------

$***$ Offline analysis \jlcmt{다시 서술 2: 백교수와 4/29 미팅 이후}

    \small
    \begin{align}
        C_i^D(0)+C_i^A(0)+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{T_i}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \le T_i
    \end{align}
    \normalsize
    
    \small
    \begin{align}
        R_i = C_i^D(0)+C_i^A(0)+B_i+\sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{R_i}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\bit)
    \end{align}
    \normalsize
    
차례대로 DA, RTA임. 무엇을 적용해도 됨. 여기서 $B_i=\max_{\tau_j\in\textsf{LP}(\tau_i)} C_j$ (또는 quantum이 1로 주어져 있으면 $C_j-1$).

% 위의 식에서 RHS-LHS를 $M_i$이라고 하자.
% 그러면 $\tau_i$는 Blocking을 $B_i+M_i$까지 받거나, 추가적인 interference를 $M_i$ 만큼 받아도 schedulable 하다.

-\\

$***$ Online analysis \jlcmt{다시 서술 2: 백교수와 4/29 미팅 이후, 작업중, 그런데, \jl{detection과 association을 한꺼번에 정하기가 어려워 보임.}}

-\\

\jlcmt{Detection 시작 시점에 $C_i^D$와 $C_i^A$ 전체에 대한 budget을 정하도록 새로운 online analysis를 만들기}

-\\

Definition. $S_i(t)$는 $\tau_i$의 $t$초에서의 state를 의미함. $S_i(t)=\textsf{DT}$는 Detection과 Association을 실행해야 할 $\tau_i$의 job이 $t$초에 존재함을 의미함. $S_i(t)=\textsf{AS}$는 (Detection은 $t$초 이전에 이미 실행하였고) Association을 실행해야 할 $\tau_i$의 job이 $t$초에 존재함을 의미함. $S_i(t)=\textsf{NO}$는 실행이 남은 $\tau_i$의 job이 $t$초에 존재하지 않음을 의미함.

-\\

Definition. $t$초나 $t$초 이후에 가장 빠른 $\tau_i$의 job release time을 $r_i(t)$라고 하자.

-\\

$\bullet$ Case-D: $\tau_i^D$가 $t$에 실행을 시작할때 (즉, $S_i(t)=\textsf{DT}$) $\tau_i^D$의 실행 시간이 $C_i^D(0)$를 뛰어넘어 얼마만큼 길어져도 되는지, 또한
$\tau_i^A$의 실행 시간이 $C_i^A(0)$를 뛰어넘어 얼마만큼 길어져도 되는지 살펴보자. 

-\\

$\bullet$ Case-D1: $\tau_i^D$와  $\tau_i^A$의 실행이 $\tau_h\in\textsf{HP}(\tau_i)$의 schedulability에 미치는 영향 계산.

$t$초에 $\tau_i^D$가 실행을 시작한다는 뜻은 모든 $S_h(t)$ 는 $\textsf{NO}$임. 

By definition, $r_i(t)$는 현재 $\tau_i$'s job의 deadline 이기도 하다. 
그러면 $r_h(t)<r_i(t)$ 인 모든 $\tau_h$에 대해서 아래의 식을 만족하면, 
$C_i^D$가 $C_i^D(0)$ 보다 커져도 $r_h(t)$에 release 하는 $\tau_h$의 job이 deadline miss 하지 않는다.

    \small
    \begin{align}
        \jl{C_i^D}+ C_h^D(0)+C_h^A(0)+\nonumber\\ \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | r_{h2}(t)<r_h(t)+T_h} \bigg\lceil\frac{r_h(t)+T_h-r_{h2}(t)}{T_{h2}}\bigg\rceil \nonumber\\\cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le T_h+\big(r_h(t)-t\bit)
    \end{align}
    \normalsize

-\\

$\bullet$ Case-D2: $\tau_i^D$의 실행시간을 증가하는 것이 $\tau_i$ 자신의 schedulaiblity에 미치는 영향 계산.

$t$초에 $\tau_i^D$가 실행을 시작한다는 뜻은 모든 $S_h(t)$ 는 $\textsf{NO}$임.

그러면 offline analysis 식은 아래와 같이 바뀐다. (이 경우 blocking은 없음)

    \small
    \begin{align}
        \jl{C_i^D+C_i^A}+ \nonumber\\ \sum_{\tau_h\in\textsf{HP}(\tau_i) | r_h(t)<r_i(t)} \bigg\lceil\frac{r_i(t)-r_h(t)}{T_h}\bigg\rceil\cdot \big(C_h^D(0)+C_h^A(0)\big) \nonumber\\
        \le r_i(t)-t
    \end{align}
    \normalsize

-\\

$\bullet$ Case-D3: $\tau_i^D$의 실행이 $\tau_j\in\textsf{LP}(\tau_i)$의 schedulability에 미치는 영향 계산.

$S_j(t)$ 가 $\textsf{DT}$, $\textsf{AS}$, $\textsf{NO}$ 인지에 따라 다르게 처리해야 하는데, 어쨋든 $\tau_j$의 job중 맨 앞에 있는 $\tau_j$의 job 하나만 고려하면 그 다음 $\tau_j$의 job 들은 고려할 필요가 없다.
그 이유는 맨 앞의 job이 schedulable 했다는 이야기는 이미 level-i busy interval이 끝나고 $\tau_j$의 실행이 되었다는 의미이므로 $C_i^D$가 커진 효과가 없다. (원래 $C_i^D(0)$ 기준 schedulability는 이미 offline에서 했으므로 OK)

1) $S_j(t)=\textsf{DT}$의 경우: \jlcmt{두번째 줄에서 $\tau_i$를 제외해야 함.}

    \small
    \begin{align}
        C_j^D(0)+C_j^A(0)+ \jl{C_i^D+C_i^A} + \nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{DT}} \big(C_{h2}^D(0)+ C_{h2}^A(0)\big) +
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{AS}} C_{h2}^A(0) + \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | t < r_{h2}(t)<r_j(t)} \bigg\lceil\frac{r_j(t)-r_{h2}(t)}{T_{h2}}\bigg\rceil\cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le r_j(t)-t
    \end{align}
    \normalsize

-\\

2) $S_j(t)=\textsf{AS}$의 경우: \jlcmt{두번째 줄에서 $\tau_i$를 제외해야 함.}

위의 식에서 $C_j^D(0)$ 만 삭제하면 됨.

-\\

3) $S_j(t)=\textsf{NO}$의 경우: \jlcmt{두번째 줄에서 $\tau_i$를 제외해야 함.}


    \small
    \begin{align}
        C_j^D(0)+C_j^A(0)+ \jl{C_i^D+C_i^A} + \nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{DT}} \big(C_{h2}^D(0)+ C_{h2}^A(0)\big) +
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | S_{h2}(t)=\textsf{AS}} C_{h2}^A(0) + \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | t < r_{h2}(t)<r_j(t)+T_j} \bigg\lceil\frac{r_j(t)+T_j-r_{h2}(t)}{T_{h2}}\bigg\rceil\nonumber\\
        \cdot \big(C_{h2}^D(0)+C_{h2}^A(0)\big) \nonumber\\
        \le T_j+\big(r_j(t)-t\big)
    \end{align}
    \normalsize

-\\

\jlcmt{Case-D1, Case-D2, Case-D3에서 나오는 모든 식들은 $\jl{C_i^D}\le constant$ \& $\jl{C_i^D+C_i^A}\le constant$의 형태이며, 모든 식을 AND 조건으로 하여 가장 tight한 식을 뽑아내면, 그것이 \jl{$C_i^D$}와 \jl{$C_i^D+C_i^A$}의 최종 constraint이다. }


-\\

$\bullet$ Case-A: $\tau_i^A$가 $t$에 실행을 시작할때 (즉, $S_i(t)=\textsf{AS}$) $\tau_i^A$의 실행 시간이 $C_i^A$를 뛰어넘어 얼마만큼 길어져도 되는지 살펴보자. 

-\\

\jlcmt{Case-A1은 Case-D1의 식에서 \jl{$C_i^D$}를 \jl{$C_i^A$}로 바꾸면 됨}

\jlcmt{Case-A2는 Case-D2의 식에서 \jl{$C_i^D+C_i^A$}를 \jl{$C_i^A$}로 바꾸면 됨}

\jlcmt{Case-A3는 Case-D3의 식에서 \jl{$C_i^D+C_i^A$}를 \jl{$C_i^A$}로 바꾸면 됨}

-\\

\jlcmt{Case-A1, Case-A2, Case-A3에서 나오는 모든 식들은 $\jl{C_i^A}\le constant$의 형태이며, 모든 식을 AND 조건으로 하여 가장 tight한 식을 뽑아내면, 그것이 \jl{$C_i^A$}의 최종 constraint이다.}

-\\

지금까지 Case-D와 Case-A를 설명했는데, 여기서 나온 조건을 바탕으로 어떻게 \jl{$C_i^D$}와  \jl{$C_i^A$}를 정할것인가?

\jlcmt{Case D에서 $\jl{C_i^D+C_i^A}\le constant$에 의해 \jl{$C_i^D$}와 \jl{$C_i^A$}의 값을 서로 조정하기는 하지만 \jl{$C_i^A$}를 크게 할당하고 이를 위해 \jl{$C_i^D$}를 작게 할당 하더라도 할당된 \jl{$C_i^A$}는 Case A 시점에 다시 체크해서 줄어들 수 있다 (늘어날 수도 있다.)
줄어들수 있는 첫번째 이유는, Case D 시점에서는 Case D1에서 higher-priority task에 대해서 \jl{$C_i^A$} 때문에 일어나는 blocking을 계산하지 않는다. 줄어들 수 있는 두번째 이유는, Case D 시점과 Case A 시점 사이에 higher-priority 작업이 실행되면서 minimum 보다 많이 실행 되었을 수 있다. 늘어날 수 있는 이유는 실행들이 WCET보다 빨리 끝나거나 interference/blocking이 패턴이 Worst보다 적기 때문이다. 

따라서 detection과 association의 tradeoff를 고려해서 Case D 시점에서 detection과 association의 시간을 주어진 detection+association budget 내에서  결정하고, 이를 Case A 시점에 association 시간을 다시 결정해야 한다.
(이것이 intra-task execution assignment임)

또한 Case D 시점에 detection+association의 upper-bound를 전부 budget으로 사용할것인지 일부만을 사용할지, 그리고 Case A 시점에 association의 upper-bound를 전부 budget으로 사용할것인지 일부만을 사용할지를 정한다. (이것이 inter-task execution assignment임)
}

~\\

\jlcmt{
그러면 inter-task 관점에서는 어떤 식으로 heuristic하게 budget을 쓸 수 있을까?

- 1. 만약 t시점에 active한 다른 job이 없으면 budget을 upper-bound 까지 모두 사용한다.

- 2. 만약 t시점에 active한 다른 작업이 있다면, 그들의 measure를 비교하여 (예: aging) 내가 가장 높으면 실행하거나, 또는 가장 높은 job의 measure minus $\alpha$ 보다 높으면 실행한다.

- 3. 2번을 만족하지 않더라도, upper-bound가 매우 커서 budget을 일부를 사용할 수 있는지를 계산해서 그만큼 실행하도록 계산한다.

}

~\\

\jlcmt{
inter-task 관점에서 budget을 정하고 나면, 그 budget 내에서 intra-task 관점에서는 어떤 식으로 heuristic하게 budget을 쓸 수 있을까?


}


-\\

Note:

\jlcmt{Case D에서 $\min_{\tau_h\in\textsf{HP}(\tau_i)}r_h(t) - C_i^D>0$이면,
$\tau_i^D$의 실행에 이어서 $\tau_i^A$의 실행이 바로 이루어지므로, 
$\tau_i^D$의 실행이 시작될 $t$ 시점에 $\tau_i^A$ 시점까지 상황까지 모두 파악이 가능함.}

-\\

Note:

\jlcmt{Offline에서는 schedulability를 높이기 위해 $\tau_i^D$와 $\tau_i^A$의 실행 사이에 preemption을 허용하지만, run-time에는 $\tau_i^D$와 $\tau_i^A$이 연달아 실행되어도 schedulability에 문제가 없을경우 그렇게 하는 방법을 생각해 볼 수 있음.}

-\\-\\-\\-\\-\\



이번 subsection에서는 이전 subsection들에서 describe된 scheduling platform과 task model을 기반으로 scheduling algorithm을 제안한다. 
우리는 주안점은 deadline miss 없이 (a) 모든 subtask의 $C_i^{D}(0)$와 $C_i^{A}(0)$ 실행을 보장하고 = critical object에 대한 accuracy를 우선적으로 maximize하고 (b) 동시에 $C_i^{D}(s_i) > C_i^{D}(0)$와 $C_i^{A}(f_i) > C_i^{A}(0)$ 실행도 최대한 해보자 =  overall accuracy도 maximize하자.
우리는 (a)와 (b)를 달성하기 위해 MOT에 특화된 property인 O3, O4를 이용하였고, GPU를 이용하는 execution의 효율성을 위해 O5도 동시에 이용하였다.
   
Object들은 대표적인 두가지 history 정보를 가지고 있다. 첫번째는 위치(location)에 대한 정보이며, 두번째는 특징(feature)에 대한 정보이다. 
MOD(multi object detection)는 사실 object의 localization과 classification의 두 작업을 수행한다. 즉 \hb{어디에 있는지} 그리고 \hb{그것이 무엇인지}.
이것이 object가 가지고 있는 가장 중요한 두 정보이다. 
MOT는 그래서 각 object의 그 두 정보를 이용하여 연속된 두 frame에 각각 존재하는 가장 유사한 두 object를 associate하는 것이다. 
따라서, MOT는 모든 object들의 이 두 정보를 저장하며 효율적으로 사용한다. 


O3에서 볼 수 있듯이 detection(e.g., DNN-based YOLO)을 매 frame마다 실행하지 않아도 MOT accuracy가 dramatic하게 떨어지지 않는 것을 볼 수 있다. 
\hbcmt{구체적인 수치 언급} 한 프레임의 detection skip은 거의 성능 변화가 없고, 몇 frame 연속으로 skip이 되어야만 성능 저하가 있다. 
이는 MOT만이 가지는 unique한 property로서, object들의 \hb{위치변화 history}를 저장하고 미래에 활용하기 때문이다. 
즉, 이전 frame에 detected된 object들의 이동경로를 활용하여 위치, 크기, 방향, 속도변화를 도출해 낼 수 있다. 
매 frame마다 detection을 하지 않아도 이정보를 이용하여 (via 칼만필터), 매우 heavy한 DNN-based detection 대비 아주 적은 computation으로 현재 frame에서의 object정보를 유추할 수 있다. 
 

O4는 MOT가 object들의 \hb{특징(feature)  history}를 저장하고 이용하기 때문이다. 
두 frame당 한번씩 feature를 전혀 뽑지 않아도 MOT accuracy 변화가 거의 없고 FPS는 비약적으로 상승한다. 
feature를 한번 뽑아 놓으면 일반적으로 최대 10 frame이 지날때까지 memory에 저장한다. 
memory의 여유에 따라 최대 100 frame까지 저장하는 경우도 있다. 
현재 frame에서 feature extraction을 했지만 전 frame에서 feature extraction을 하지 않았더라도 그전 frame에서 뽑아 놓은 object들의 feature와 비교하여 가장 높은 유사도를 가지는 object와 연결짓는다. 즉, 그 object의 ID를 할당한다. 
하지만, O3와 O4에서 볼 수 있는 MOT의 이러한 object에 대한 정보도 여러 frame이 지나면 information vanishing 현상을 겪으면서 부정확해 질 수 있다.
  

O5는 MC-MOT의 Detection에서 total image size가 8가지로 변할때, Association에서 object수의 구간이 8가지로 변할때, 걸리는 시간을 나타내는 것이다(\hbcmt{accuracy변화도 보여줄 수 있나? 보여줘야 하나?}).
O5에서 볼 수 있듯이, detection에서 total image size가 0일때와 그다음 size일때 걸리는 시간이 비약적으로 늘어난다. 
이것은 해당 inference연산이 GPU를 이용한 연산이므로, 약간이라도 연산을 할때 GPU를 호출하는 비용이 들기 때문이다.
association에서도 같은 현상이 일어난다. 
feature는 하나라도 뽑게 되면, GPU를 호출하기 위한 비용이 발생하게 된다. 
따라서, 이러한 GPU호출의 비싼 최소비용을 고려해 보았을때, 한번 GPU 호출을 하게 되면 충분한 workload를 실행시켜야 한다. 

%\hbcmt{$\tau_i^A$의 job이 $\tau_i$의 release에서 release되는지, }

O3, O4, O5를 고려해 보았을때, Detection과 Association이 매순간 fully 실행 될 필요는 없으며 (from O3, O4), 같은 computation resource가 충분하지 않을 경우 한쪽에 몰아주는 것이 더 computational effective하다는 결론을 얻는다.  

Based on the reasoning, we propose two scheduling algorithms called EDF-Flexible and EDF-Aging.
As described in the previous section, the tasks under the proposed algorithms are executed non-preemptively. 
A scheduling decision can be made at every release and completion of each subtask, $\tau_i^{D}$ and $\tau^{A}$. 
As EDF-Flexible and EDF-Aging are based on EDF, each job of $\tau_i^{D}$ or $\tau_i^{A}$ with the earliest absolute deadline has the highest priority. 
두 스케줄링 모두 각각의 (a)와 (b)를 만족시키기 위해, policy에 따라 $\tau_i^{D}$ and $\tau^{A}$의 worst-case execution time을 동적으로 변화시킨다.  

-\\

\newpage

\jlcmt{2022.5.14 20:00 백형부 교수와 미팅:

$C_i^D$ and $C_i^A$ 는 preemption 없이 전체가 non-preemptive 로 동작한다.

$C_i$가 실행되기 직전에 active한 모든 job의 online analysis를 돌려서 가능한 실행 선택지(priority-inversion으로 실행해도 모두가 schedulable한)를 system 전달하고, 
system은 주어진 measure를 계산해서 object reliability가 가장 많이 증가하는 선택지를 고른다.

이것을 반영할 수 있는 analysis를 다시 정리.

min/min, min/max, max/min, max/max

}



\subsection{Offline analysis}

    \small
    \begin{align}
        R_i = C_i^\texttt{min}+max_{\tau_j\in \textsf{LP}(\tau_i)} C_j^\texttt{min} + \sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{R_i}{T_h}\bigg\rceil\cdot C_h^\texttt{min}
    \end{align}
    \normalsize
    
증명: 

$\tau_i$의 job의 release 시점에 execution이 남아있는 higher-priority task의 job이 없으면,
이경우는 blocking이 없음. 이것은 preemptive FP에서 sync release가 critical instant가 됨으로 증명된다. 

그러면 blocking이 있는 경우를 따져 봐야 함. $\tau_i$의 job의 release 시점 직전에 blocking이 job이 시작된것이 아니라면, $\tau_i$의 job의 release를 더 이전으로 당기는것이 response time이 늘어난다. 따라서 blocking이 직전에 일어나고 higher-priority job 이 sync release 인경우가 response time이 최대이며, 위의 식으로 그러한 상황의 response time을 계산하고 있으므로 worst-case response time이다.

\subsection{Online analysis without priority-inversion}


Definition. $A_i(t)$는 $\tau_i$의 $t$초에서의 activeness를 의미함. $A_i(t)=\textsf{T}$는 
실행해야 할 $\tau_i$의 job이 $t$초에 존재함을 의미함.
$A_i(t)=\textsf{F}$는 실행이 남은 $\tau_i$의 job이 $t$초에 존재하지 않음을 의미함.

-\\

Definition. $t$초나 $t$초 이후에 가장 빠른 $\tau_i$의 job release time을 $r_i(t)$라고 하자.

-\\

$\tau_i$의 job이 실행을 시작할 시점이 되었을때 $\tau_i$의 실행시간 $C_i$가 $C_i^\texttt{min}$을 뛰어넘어
얼마만큼 길어져도 되는지 살펴보자. 
즉, $C_i$는 (detection, association)에 대해 (max, min), (min, max), (max, max) 3가지에 대해 실행이 가능한지 살펴봐야 한다. offline analysis에 의해 (min, min)의 실행은 online analysis를 해보지 않아도 이미 보장된다.


-\\

$\bullet$ Case1: $\tau_i$의 실행시간을 증가하는 것이 $\tau_i$ 자신의 schedulability에 미치는 영향 계산.

-\\

non-preemptive이므로 간단함.
By definition, $r_i(t)$는 현재 $\tau_i$'s job의 deadline 이기도 하다. 

-\\

그러면 offline analysis 식은 아래와 같이 바뀐다. (이 경우 blocking은 없음)

    \small
    \begin{align}
        C_i \le r_i(t)-t
    \end{align}
    \normalsize

-\\

$\bullet$ Case2: $\tau_i$의 실행이 $\tau_h\in\textsf{HP}(\tau_i)$의 schedulability에 미치는 영향 계산.

-\\

$t$초에 $\tau_i$가 실행을 시작한다는 뜻은 모든 $A_h(t)=\textsf{F}$임. 

-\\

By definition, $r_i(t)$는 현재 $\tau_i$'s job의 deadline 이기도 하다. 
그러면 $r_h(t)<r_i(t)$ 인 모든 $\tau_h$에 대해서 아래의 식을 만족하면, 
$C_i$가 $C_i^\texttt{min}$ 보다 커져도 $r_h(t)$에 release 하는 $\tau_h$의 job이 deadline miss 하지 않는다.

    \small
    \begin{align}
        C_i+ C_h^\texttt{min}+\nonumber\\ \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | r_{h2}(t)<r_h(t)+T_h} \bigg\lceil\frac{r_h(t)+T_h-r_{h2}(t)}{T_{h2}}\bigg\rceil \cdot C_{h2}^\texttt{min} \nonumber\\
        \le r_h(t)+T_h-t
    \end{align}
    \normalsize

-\\


위의 analysis는 $\tau_h$의 release 부터 보지 않고, t부터 $\tau_h$의 deadline까지를 보게 된다.
만약에 중간에 idle한 t'이 있다면, t' 부터는 $\tau_i$의 $C_i$가 늘어나서 생기는 효과가 없어지므로 
이 경우는 offline analysis에서 이미 커버되므로 신경쓰지 않아도 된다.
즉, 위의 analysis는 $C_i$가 커지는 효과가 계속 영향을 미쳐서 혹시 이후에 release하는 $\tau_h$의 job이
unschedulable 한지를 살펴보는 것이다. 

\jlcmt{왜 $\tau_h$의 다음다음 job의 schedulability는 살펴보지 않아도 되나?}
이번 $\tau_h$의 job과 다음 $\tau_h$의 job 사이에 $\tau_h$보다 priority 높은 job의 실행이 없으면 다음 $\tau_h$의 job의 상황은 offline analysis로 커버된다.
이번 $\tau_h$의 job과 다음 $\tau_h$의 job 사이에 $\tau_h$보다 priority 높은 $\tau_{h2}$의 job의 실행이 있으면, $\tau_{h2}$의 job 입장에서 이번 $\tau_h$의 job의 실행은 blocking으로 작용할 수 있는데 이번 $\tau_h$의 job의 실행은 minimum 실행이므로 offline analysis로 커버된다.

-\\


$\bullet$ Case3: $\tau_i$의 실행이 $\tau_j\in\textsf{LP}(\tau_i)$의 schedulability에 미치는 영향 계산.

$A_j(t)$ 가 $\textsf{T}$ 인지 $\textsf{F}$ 인지에 따라 다르게 처리해야 하는데, 어쨋든 $\tau_j$의 job중 맨 앞에 있는 $\tau_j$의 job 하나만 고려하면 그 다음 $\tau_j$의 job 들은 고려할 필요가 없다.
그 이유는 맨 앞의 job이 schedulable 했다는 이야기는 이미 level-i busy interval이 끝나고 $\tau_j$의 실행이 되었다는 의미이므로 $C_i$가 커진 효과가 없다. (원래 $C_i$ 기준 schedulability는 이미 offline에서 했으므로 OK)

\jlcmt{왜 다음 job만 고려하면 되나?}

1) $A_j(t)=\textsf{T}$의 경우: %\jlcmt{두번째 줄에서 $\tau_i$를 제외해야 함.}

    \small
    \begin{align}
        C_j^\texttt{min}+ C_i + 
        \sum_{\tau_{h2}\neq\tau_i\in\textsf{HP}(\tau_j) | A_{h2}(t)=\textsf{T}} C_{h2}^\texttt{min}+\nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | r_{h2}(t)<r_j(t)} \bigg\lceil\frac{r_j(t)-r_{h2}(t)}{T_{h2}}\bigg\rceil\cdot C_{h2}^\texttt{min} \nonumber\\
        \le r_j(t)-t
    \end{align}
    \normalsize

-\\

2) $A_j(t)=\textsf{F}$의 경우: %\jlcmt{두번째 줄에서 $\tau_i$를 제외해야 함.}


    \small
    \begin{align}
        C_j^\texttt{min} +C_i + 
        \sum_{\tau_{h2}\neq \tau_i\in\textsf{HP}(\tau_j) | A_{h2}(t)=\textsf{T}} C_{h2}^\texttt{min} +
        \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | r_{h2}(t)<r_j(t)+T_j} \bigg\lceil\frac{r_j(t)+T_j-r_{h2}(t)}{T_{h2}}\bigg\rceil    \cdot C_{h2}^\texttt{min} \nonumber\\
        \le r_j(t)+T_j-t
    \end{align}
    \normalsize

-\\


\subsection{Online analysis with priority-inversion}

$\tau_i$의 job이 실행을 시작할 시점이 되었을때, $\tau_i$의 job 뿐만 아니라, $A_k(t)=\texttt{T}$를 만족하는 모든  $\tau_k$ (사실 $\tau_k\in \textsf{LP}(\tau_i)$)에 대해서 얼마만큼 실행이 가능한지 계산한다. 
즉, $C_i$ for $\tau_i$는 (detection, association)에 대해 (max, min), (min, max), (max, max) 3가지에 대해 실행이 가능한지 살펴봐야 한다. offline analysis에 의해 (min, min)의 실행은 online analysis를 해보지 않아도 이미 보장된다. 이 모든 경우는 이전 subsection과 동일하게 진행한다.

마찬가지로 $C_k$ for $\tau_k$도 (detection, association)에 대해 (max, min), (min, max), (max, max) 3가지에 대해 실행이 가능한지 살펴봐야 한다. (min, min)만 가능하면 $\tau_k$를 실행하지 않을 것이기 때문에 실행 가능한지 살펴볼 필요가 없다. 지금부터 $\tau_k$를 priority-inversion에 의해 $\tau_i$ 대신 실행했을때 sch edulability를 살펴보자. 이 때 $\tau_k$의 실행이후의 다른 모든 작업들은 min으로 원래 priority에 맞춰 실행할 상황을 고려한다.

-\\

$\bullet$ Case1: $\tau_k$의 실행이 증가하는 것이 $\tau_k$ 자신의 schedulability에 미치는 영향 계산.

-\\


non-preemptive이므로 간단함.
By definition, $r_i(t)$는 현재 $\tau_i$'s job의 deadline 이기도 하다. 

-\\

그러면 offline analysis 식은 아래와 같이 바뀐다. (이 경우 blocking은 없음)

    \small
    \begin{align}
        C_k \le r_k(t)-t
    \end{align}
    \normalsize

-\\

$\bullet$ Case2: $\tau_k$의 실행이 $\tau_h\in\textsf{HP}(\tau_k)$의 schedulability에 미치는 영향 계산.

-\\

$t$초에 $\tau_k$가 실행을 시작하더라도 priority-inversion을 허용하므로 $A_h(t)=\textsf{T}$와 $\textsf{F}$가  모두 가능함.

-\\

1) $A_h(t)=\textsf{T}$:


By definition, $r_h(t)$는 현재 $A_h(t)=\texttt{T}$인 $\tau_h$'s job의 deadline 이기도 하다. 
%그러면 $r_h(t)<r_k(t)$ 인 모든 
$A_h(t)=\textsf{T}$인 모든 $\tau_h$에 대해서 아래의 식을 만족하면, 
$C_k$가 $C_k^\texttt{min}$ 보다 커져도 현재 active한  $\tau_h$의 job이 deadline miss 하지 않는다.

    \small
    \begin{align}
        C_k+C_h^\texttt{min} + 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | A_{h2}(t)=\texttt{T}} C_{h2}^\texttt{min} + \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | %A_{h2}(t)=\texttt{F} ~\&~ 
        r_{h2}(t)<r_h(t) } \bigg\lceil\frac{r_h(t)-r_{h2}(t)}{T_{h2}}\bigg\rceil \cdot C_{h2}^\texttt{min} \nonumber\\
        \le r_h(t)-t
    \end{align}
    \normalsize

-\\

\jlcmt{왜 다음 job만 고려하면 되나?}

-\\

2) $A_h(t)=\textsf{F}$:

By definition, $r_h(t)+D_h$는 현재 $A_h(t)=\texttt{F}$인 $\tau_h$의 다음 release될 job의 deadline 이다.
%그러면 $r_h(t)<r_k(t)$ 인 모든 
$A_h(t)=\textsf{F}$인 모든 $\tau_h$에 대해서 아래의 식을 만족하면, 
$C_k$가 $C_k^\texttt{min}$ 보다 커져도 다음 release 될 $\tau_h$의 job이 deadline miss 하지 않는다.


    \small
    \begin{align}
        C_k+C_h^\texttt{min} + 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | A_h(t)=\texttt{T}} C_{h2}^\texttt{min} + \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_h) | A_h(t)=\texttt{F} ~\&~ r_{h2}(t)<r_h(t)+T_h } \bigg\lceil\frac{r_h(t)+T_h-r_{h2}(t)}{T_{h2}}\bigg\rceil \cdot C_{h2}^\texttt{min} \nonumber\\
        \le r_h(t)+T_h-t
    \end{align}
    \normalsize


\jlcmt{왜 다음 job만 고려하면 되나?}

-\\



$\bullet$ Case3: $\tau_k$의 실행이 $\tau_j\in\textsf{LP}(\tau_k)$의 schedulability에 미치는 영향 계산.
(no priority-inversion의 $\tau_i$ 부분을 $\tau_k$로만 고치면 됨)

$A_j(t)$ 가 $\textsf{T}$ 인지 $\textsf{F}$ 인지에 따라 다르게 처리해야 하는데, 어쨋든 $\tau_j$의 job중 맨 앞에 있는 $\tau_j$의 job 하나만 고려하면 그 다음 $\tau_j$의 job 들은 고려할 필요가 없다.
그 이유는 맨 앞의 job이 schedulable 했다는 이야기는 이미 level-i busy interval이 끝나고 $\tau_j$의 실행이 되었다는 의미이므로 $C_i$가 커진 효과가 없다. (원래 $C_i$ 기준 schedulability는 이미 offline에서 했으므로 OK)
\jlcmt{이게 priority-inversion인 경우도 되는건가?}

1) $A_j(t)=\textsf{T}$의 경우: %\jlcmt{두번째 줄에서 $\tau_i$를 제외해야 함.}

    \small
    \begin{align}
        C_j^\texttt{min}+ C_k + 
        \sum_{\tau_{h2}\neq\tau_k\in\textsf{HP}(\tau_j) | A_{h2}(t)=\textsf{T}} C_{h2}^\texttt{min}+\nonumber\\ 
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | r_{h2}(t)<r_j(t)} \bigg\lceil\frac{r_j(t)-r_{h2}(t)}{T_{h2}}\bigg\rceil\cdot C_{h2}^\texttt{min} \nonumber\\
        \le r_j(t)-t
    \end{align}
    \normalsize

-\\

2) $A_j(t)=\textsf{F}$의 경우: %\jlcmt{두번째 줄에서 $\tau_i$를 제외해야 함.}


    \small
    \begin{align}
        C_j^\texttt{min} +C_k + 
        \sum_{\tau_{h2}\neq \tau_k\in\textsf{HP}(\tau_j) | A_{h2}(t)=\textsf{T}} C_{h2}^\texttt{min} +
        \nonumber\\
        \sum_{\tau_{h2}\in\textsf{HP}(\tau_j) | r_{h2}(t)<r_j(t)+T_j} \bigg\lceil\frac{r_j(t)+T_j-r_{h2}(t)}{T_{h2}}\bigg\rceil    \cdot C_{h2}^\texttt{min} \nonumber\\
        \le r_j(t)+T_j-t
    \end{align}
    \normalsize

-\\

\subsection{Online analysis를 할때 offline analysis로 커버되어 schedulability를 따져보지 않아도 되는 상황}

$\bullet$ blocking:

내가  $\tau_h$의 job인데, 내가 lower-priority 작업에 의해 blocking 되었고, blocking을 하게된 작업이 시작할때 $\tau_h$ 보다 높은 priority의 active 작업이 없었음. 그리고 그 lower-priority 작업은 min으로 동작함.

이 상황을 만나면 $\tau_h$의 job의 schedulability는 offline analysis에 의해 보장.

-\\

$\bullet$ no blocking but interference: (밑에 정리가 있으면 필요없음)

내가  $\tau_h$의 job인데, 나의 release 시점부터 a job of higher-priority task $\tau_{h2}$에 의해 interference를 받음. 

그러면 the job of $\tau_{h2}$를 거꾸로 따라갔을때, 그 작업이 위의 blocking을 조건을 만족하면 $\tau_{h2}$의 job의 schedulability가 offline analysis에 의해 보장되며, 이어서 $\tau_h$의 job의 schedulability도 offline analysis에 의해 보장됨.

-\\

$\bullet$ 정리: $C_i$가 $C_i^\texttt{min}$에 비해 늘어났거나 priority-inversion이 일어난 마지막 시점을 $t$라고 하자. 그러면 $t$ 이후에 어떤 job이 위의 blocking 조건을 만족하면, blocking이 일어난 job과 이후에 실행하는 모든 job의 schedulability는 이후에 $C_i$가 $C_i^\texttt{min}$에 비해 늘어났거나 priority-inversion이 다시 일어나기 전까지는 offline analysis에 의해 보장된다.


\newpage

\section{New Analysis}

\subsection{Offline analysis}

    \small
    \begin{align}
        R_i = C_i^\texttt{min}+max_{\tau_j\in \textsf{LP}(\tau_i)} C_j^\texttt{min} + \sum_{\tau_h\in\textsf{HP}(\tau_i)} \bigg\lceil\frac{R_i}{T_h}\bigg\rceil\cdot C_h^\texttt{min}
    \end{align}
    \normalsize
    
증명: 

$\tau_i$의 job의 release 시점에 execution이 남아있는 higher-priority task의 job이 없으면,
이경우는 blocking이 없음. 이것은 preemptive FP에서 sync release가 critical instant가 됨으로 증명된다. 

그러면 blocking이 있는 경우를 따져 봐야 함. $\tau_i$의 job의 release 시점 직전에 blocking이 job이 시작된것이 아니라면, $\tau_i$의 job의 release를 더 이전으로 당기는것이 response time이 늘어난다. 따라서 blocking이 직전에 일어나고 higher-priority job 이 sync release 인경우가 response time이 최대이며, 위의 식으로 그러한 상황의 response time을 계산하고 있으므로 worst-case response time이다.

\subsection{Online analysis with/without priority-inversion}

Definition. $A_i(t)$는 $\tau_i$의 $t$초에서의 activeness를 의미함. $A_i(t)=\textsf{T}$는 
실행해야 할 $\tau_i$의 job이 $t$초에 존재함을 의미함.
$A_i(t)=\textsf{F}$는 실행이 남은 $\tau_i$의 job이 $t$초에 존재하지 않음을 의미함.

-\\

Definition. $t$초나 $t$초 이후에 가장 빠른 $\tau_i$의 job release time을 $r_i(t)$라고 하자.

-\\

$\tau_i$의 job이 실행을 시작할 시점이 되었을때 $\tau_i$의 실행시간 $C_i$가 $C_i^\texttt{min}$을 뛰어넘어
얼마만큼 길어져도 되는지 살펴보자. 
즉, $C_i$는 (detection, association)에 대해 (max, min), (min, max), (max, max) 3가지에 대해 실행이 가능한지 살펴봐야 한다. offline analysis에 의해 (min, min)의 실행은 online analysis를 해보지 않아도 이미 보장된다.

-\\

At $t$: 어떤 job의 작업 실행이 끝나거나, cpu가 idle한 상태에서 at least one job이 $t$에 release 함.

이때 FP의 priority와 "관계없이" $\tau_k$를 $C_k$만큼 ($C_k^\texttt{min}$을 넘어서서) $t$에서 실행하고 이후 job 들은 "모두" FP의 priority 대로 min 만큼 실행되었을때 $t$ 이후에 실행되는 모든 task $\tau_j\in\tau$의 다음 한개의 job이 schedulable 한지는 아래와 같이 판단한다. 

-\\



$\bullet$ Case 1: $A_j(t)=\textsf{T}$인 $\tau_j$ ($\neq \tau_k$)의 schedulability

-\\

    \small
    \begin{align}
        C_j^\texttt{min} + C_k+
        \sum_{\tau_{h}\in\textsf{HP}(\tau_j)\setminus\{\tau_k\} | A_{h}(t)=\textsf{T}} C_{h}^\texttt{min} + \nonumber\\
        \sum_{\tau_{h}\in\textsf{HP}(\tau_j) | %A_{h2}(t)=\texttt{F} ~\&~ 
        r_h(t)<r_j(t) } \bigg\lceil\frac{r_j(t)-r_h(t)}{T_h}\bigg\rceil \cdot C_h^\texttt{min} \nonumber\\
        \le r_j(t)-t
    \end{align}
    \normalsize

-\\


$\bullet$ Case 2: $A_j(t)=\textsf{F}$인 $\tau_j$ ($\neq \tau_k$)의 schedulability

-\\

    \small
    \begin{align}
        C_j^\texttt{min} + C_k+
        \sum_{\tau_{h}\in\textsf{HP}(\tau_j)\setminus\{\tau_k\} | A_{h}(t)=\textsf{T}} C_{h}^\texttt{min} + \nonumber\\
        \sum_{\tau_{h}\in\textsf{HP}(\tau_j) | %A_{h2}(t)=\texttt{F} ~\&~ 
        r_h(t)<r_j(t)+T_j } \bigg\lceil\frac{r_j(t)+T_j-r_h(t)}{T_h}\bigg\rceil \cdot C_h^\texttt{min} \nonumber\\
        \le r_j(t)+T_j-t
    \end{align}
    \normalsize

-\\

$\bullet$ Case 3: $\tau_j=\tau_k$의 schedulability

$\bullet$ Case 3-1: $\tau_j=\tau_k$의 지금 실행될 job


-\\

    \small
    \begin{align}
        C_k \le r_k(t)-t
    \end{align}
    \normalsize

-\\

$\bullet$ Case 3-2: $\tau_j=\tau_k$의 지금 실행될 다음 job (왜 다음 job까지 해야 하는 지는 다음 subsection의 theorem 참고)

-\\

   Case 2식에서 j index를 모두 k로 바꾸면 됨.

-\\

\subsection{그럼 이전 subsection을 써서 어떻게 online schedulability를 guarantee 하는가?}

이전 subsection에서 모든 task의 다음 job 한개씩의 schedulability를 guarantee했다.

이전 subsection 서술: (이때 FP의 priority와 "관계없이" $\tau_k$를 $C_k$만큼 ($C_k^\texttt{min}$을 넘어서서) $t$에서 실행하고 이후 job 들은 "모두" FP의 priority 대로 min 만큼 실행되었을때 $t$ 이후에 실행되는 모든 task $\tau_h\in\tau$의 다음 한개의 job이 schedulable 한지는 아래와 같이 판단한다. )

-\\

그러면 이것이 어떻게 task 당 한개의 job 다음 job들까지의 schedulability를 보장할 것인가?

-\\


Lemma. (blocking means offline schedulability)
내가  $\tau_j$의 job인데, 내가 lower-priority 작업에 의해 blocking 되었고, blocking을 하게된 작업이 시작할때 $\tau_j$ 보다 높은 priority의 active 작업이 없었음. 그리고 그 lower-priority 작업은 min으로 동작함.
이 상황을 만나면 $\tau_j$의 job의 schedulability는 offline analysis에 의해 보장.

-\\

Lemma. (no blocking and higher-priority carry-in means offline schedulability)
내가  $\tau_j$의 job인데, release 시점에 blocking도 없고 higher-priority carry-in job도 없음.
이 상황을 만나면 $\tau_j$의 job의 schedulability는 offline analysis에 의해 보장.

-\\

Theorem. (위의 두 lemma의 일반화) priority를 지키지않았거나 execution이 min보다 늘어난 마지막 시점 이후에 level-$j^+$ idle time ($\tau_j$ 보다 priority가 높은 active job이 없는 시간)이 있으면 이후의 $\tau_j$의 job은 offline analysis에 의해 schedulable가 보장됨.

이 Theorem 때문에 Case 3-2를 해야 함. (Case 3-1은 priroity를 지키지 않았거나 execution이 min보다 늘어난 당사자임)

-\\

Theorem. 위의 theorem에 의해서, 만약 $\tau_j$의 다음 job의 실행이 되었다는 것은 level-$j^+$ idle time이 생겼으므로 $\tau_j$의 다음다음 job 이후 job은 항상 schedulable 하다.
%과 다음다음 job의 실행 사이에 level-j idle time이 있다면, 다음다음 job은 자동으로 schedulable함.
%만약 $\tau_j$의 다음 job의 실행과 다음다음 job의 실행 사이에 level-j idle time이 없다면,





-\\




\newpage

\section{OLD}

\subsection{Scheduling Policy}

We design scheduling policies specialized for RT-MOT, which satisfies (i) \jl{the minimum degree} of execution of every sub-job of $\tau_i^D$ and $\tau_i^A$ (corresponding to $C_i^D(0)$ and $C_i^A(0)$ for every $\tau_i\in\tau$ should finished within its deadline, and 
(ii) \jlcmt{minimum 이상의 execution을 deadline miss 없이 실행하되, critical object 및 overall accuracy가 올라가는 방향으로 어떤 작업의 어떤 서브작업을 어느 degree로 실행할지 결정한다.}
For (i), we apply EDF (Earliest Deadline First)~\cite{LiLa73} as an underlying prioritization policy.
Suppose that we always execute \jl{the minimum degree} of execution of every sub-job of $\tau_i^D$ and $\tau_i^A$ for every $\tau_i\in\tau$.
Then, the execution of every sub-job is finished within its deadline, if the following inequality holds (derived from \cite{Bak90,KCK22}).
%Then, similar to \cite{KCK22}, 

\noindent
\begin{lemma}\label{lemma:schedulability}
If the following inequality holds, then $\tau$ \jl{with the minimum degree} is schedulable by 

\noindent \small
\begin{align} \label{eq:schedulablility}
\frac{\max_{\tau_i \in \tau}\jl{\max\big(C_i^{D}(0),C_i^{A}(0)\big)}}{\min_{\tau_i \in \tau} T_i} + \sum_{\tau_i \in \tau} \frac{C_i^{D}(0)+C_i^{A}(0)}{T_i} \le 1.0.
\end{align}
\normalsize
%\jlcmt{사실 첫번째 term은 max (CD+CA)/min T 가 아니라 max (max(CD, CA))/min T 로 더 tight함. (이것을  반영하여 새로 구현하는게 좋을지?}
\end{lemma}
\begin{proof}
\hb{proof here}
~\\~\\~\\
~\\~\\~\\
~\\~\\~\\
~\\~\\~\\
~\\~\\~\\
~\\~\\~\\
\end{proof}

We design two scheduling policies that preserves Lemma~\ref{lemma:schedulability} while satisfying (i) and (ii): EDF-BE (Best Effort) and EDF-Aging.
\jlcmt{여기에 각 작업은 $\tau_i^D$ 실행이 끝나고, $\tau_i^A$가 실행되며 각 sub-job은 non-preemptive이지만, $\tau_i^D$와 $\tau_i^A$의 실행사이는 preemptable임을 설명\\}


\textbf{EDF-BE.} 
To achieve (i) and (ii), the simplest way is to prioritize \jl{the minimum degree of execution} of every sub-job and perform \jl{the execution beyond the minimum degree} only if there is no sub-job with remaining execution for the minimum degree.
This is implemented by EDF-BE (Best Effort) explained as follows.
Every sub-job is scheduled by EDF.
When a sub-job of $\tau_i^D$ is selected to be executed at $t_{cur}$,
it determines the execution degree of itself (i.e., $\tau_i^D$) and its corresponding association sub-job (i.e., $\tau_i^A$).
If there is other active job at $t_{cur}$ than $\tau_i^D$, 
the execution degree for $\tau_i^D$ and that of $\tau_i^A$ are set to the minimum (i.e., $C_i^D(0)$ and $C_i^A(0)$);
otherwise, \jlcmt{$f_i$는 0으로 세팅되고,  $s_i$는 본인이 가질 수 있는 8가지의 값 중 $C_i^{D}(s_i) + C_i^{A}(0) \le d_1(t_{cur}) - t_{cur}$를 만족하는 가장 큰 값으로 세팅되며, 
$m_i$는 $M_i^{A}$이 된다. 
If $m_i = M_i^{A}$, $s_i$는 0으로 세팅되고,  $f_i$는 본인이 가질 수 있는 8가지의 값 중 $C_i^{D}(0) + C_i^{A}(f_i) \le d_1(t_{cur}) - t_{cur}$를 만족하는 가장 큰 값으로 세팅되며, 
$m_i$는 $M_i^{D}$이 된다. \\}
EDF-BE satisfies (i) in that First, the minimum degree of execution of every sub-job of $\tau_i^D$ and $\tau_i^A$ is not delayed by any execution beyond the minimum degree.
\jlcmt{왜 (ii)를 partially support하는가? (optional 작업의 schedulability를 포함해서)\\}
Therefore, Eq.~\eqref{eq:schedulablility} can be a schedulability test for EDF-BE.



\begin{algorithm}[t!] \jlcmt{수정 필요} %\hbcmt{should be modified}
	\caption{\small EDF-Aging: scale decision for $\tau_i^{D}$ and $\tau_i^{A}$ at $t_{cur}$}
	\label{algo:aging}
	\small
	\begin{algorithmic}[1]
		\STATE $p$=0, $U^M$ = the left-hand-side of Eq.~\eqref{eq:schedulablility}		
		\FOR {$i$ = $n$ to 1, $\tau_i^{D}$ $\in$ $\{\tau_1^D, ..., \tau_n^D|d_1(t_{cur}, \le, \cdots \le d_n(t_{cur})\}$}
		\STATE $U^M$ = $U^M$ - $\frac{\tau_i^D(0)+\tau_i^A(0)}{T_i}$
		\STATE $q_i$ = $max(0, RC_i^0 - (1-U^M)\dot (d_i(t_{cur}-d_1(t_{cur}))))$ 
		\STATE $U^M$ = $min(1.0, U^M+ \frac{d_i(t_{cur} - d_1(t_{cur}))}{RC_i^0-q_i})$
		\STATE $p$ = $p + q_i$
		\ENDFOR
		\STATE  $Slack(t_{cur}, d_1(t_{cur})) $ = $d_1(t_{cur}) - t_{cur} - p$
		\STATE \textbf{return} arg $\max_{s_k \in S_k}\{C_k^D(s_k)|C_k\}$
	\end{algorithmic}
	\normalsize
\end{algorithm}

\textbf{EDF-BE$^+$.}
\jlcmt{EDF-BE와 기본적으로 같은 방법인데, 본인이 가질수 있는 execution degree 중 가장 높은 것을 고르도록 시간을 계산할때, minimum degree의 execution을 delay 시켜서 그들을 schedulable 하게 할 수 있다면 이를 고려해서 계산함. \cite{KCK22}의 EDF-slack 구조를 가져옴.\\}

\jlcmt{Algorithm~1을 서술하고 설명.\\-\\-\\}

\jlcmt{왜 (i)와 (ii)를 만족하는가, Eq.~\eqref{eq:schedulablility} can be a schedulability test for EDF-BE$+$.\\-\\-\\}


\textbf{EDF-Aging.}
We apply the same structure as EDF-BE$^+$ in terms of calculating the amount of time that a sub-job of $\tau_i^D$ and that of $\tau_i^A$ can utilize.
However, we develop a more systematic way to determine how to distribute the amount of time \jl{not only to sub-jobs of different tasks, but also to the sub-jobs within the same task.}
To this end, 
we utilize the concept of \textit{aging}.
\jlcmt{우리 scheduling에서의 aging의 개념 및 이것이 왜 (ii) 달성에 효과적인지 설명\\-\\-\\}
\jlcmt{general 하게 설명 $\alpha$, $\beta$ 등으로 parameterize하고, 적절한 값은 evaluation에서 empirical하게 찾음.\\-\\-\\}
\jlcmt{왜 (i)와 (ii)를 만족하는가, Eq.~\eqref{eq:schedulablility} can be a schedulability test for EDF-Aging.\\-\\-\\}

% -------------

% \subsection{EDF-Flexible}

% EDF-Flexible(\hbcmt{naive version})은 모든 subtask의 $C_i^{D}(0)$와 $C_i^{A}(0)$ 실행이 받는 interference를 최소화 시키기 위한 방법이다. 
% Recall that EDF-Flexible is based on EDF, and thus a job with an earliest deadline has the highest priority. 
% EDF-Flexible은 매 $\tau_i^{D}$의 job이 실행을 시작할때 $s_i$ 와 $f_i$의 크기를 결정하고, $C_i^{D}(s_i)$와 $C_i^{A}(f_i)$는 결정 된 $s_i$ 와 $f_i$에 의해 자연스럽게 결정된다.
% 또한, mode $m_i \in M_i = {M_i^{D}, M_i^{A}}$를 가지는데, $m_i$는 처음에 $M_i^{D}$로 세팅된다. 
% Let $t_{cur}$와 $d_i(t_{cur})$를 현재시간과 현재시간에서 가장 빠른 i번째 absolute deadline이라고 하자.  
% \hbcmt{Algorithm 박스 만들어야 할지?}
% A job of $\tau_i^{D}$가 어떠한 시간 $t_{cur}$에서 실행을 시작할 때, 두가지 상황을 고려한다:
% (i) only two jobs of $\tau_i^{D}$ and $\tau_i^{A}$ are active, 
% and (ii) another job of $\tau_j \neq \tau_i$ is active. 
% In (i), if $m_i = M_i^{D}$, $f_i$는 0으로 세팅되고,  $s_i$는 본인이 가질 수 있는 8가지의 값 중 $C_i^{D}(s_i) + C_i^{A}(0) \le d_1(t_{cur}) - t_{cur}$를 만족하는 가장 큰 값으로 세팅되며, 
% $m_i$는 $M_i^{A}$이 된다. 
% If $m_i = M_i^{A}$, $s_i$는 0으로 세팅되고,  $f_i$는 본인이 가질 수 있는 8가지의 값 중 $C_i^{D}(0) + C_i^{A}(f_i) \le d_1(t_{cur}) - t_{cur}$를 만족하는 가장 큰 값으로 세팅되며, 
% $m_i$는 $M_i^{D}$이 된다. 
% In (ii), $s_i$ and $f_i$ are set to zero, and $m_i$ is not changed.
% ~~\\~~\\~~\\
% ~~\\~~\\~~\\
% \hbcmt{exmaple과 figure필요}
% ~~\\~~\\~~\\
% ~~\\~~\\~~\\

% \noindent
% \begin{theorem}
% If the following equation holds, then $\tau$ is schedulable by EDF-Flexible
% \begin{align} \label{eq:schedulable}
% \frac{\max_{\tau_i \in \tau}(C_i^{D}(0)+C_i^{A}(0))}{\min_{\tau_i \in \tau} T_i} + \sum_{\tau_i \in \tau} \frac{C_i^{D}(0)+C_i^{A}(0)}{T_i} \le 1.0    
% \end{align}

% \jlcmt{사실 첫번째 term은 max (CD+CA)/min T 가 아니라 max (max(CD, CA))/min T 로 더 tight함. (이것을  반영하여 새로 구현하는게 좋을지?}
% \end{theorem}
% \begin{proof}
% \hb{proof here}
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% \end{proof}



% \subsection{EDF-Aging}

% \begin{algorithm}[t!] \hbcmt{should be modified}
% 	\caption{\small EDF-Aging: scale decision for $\tau_i^{D}$ and $\tau_i^{A}$ at $t_{cur}$}
% 	\label{algo:aging}
% 	\small
% 	\begin{algorithmic}[1]
% 		\STATE $p$=0, $U^M$ = the left-hand-side of Equation~\eqref{eq:schedulable}		
% 		\FOR {$i$ = $n$ to 1, $\tau_i^{D}$ $\in$ $\{\tau_1^D, ..., \tau_n^D|d_1(t_{cur}, \le, \cdots \le d_n(t_{cur})\}$}
% 		\STATE $U^M$ = $U^M$ - $\frac{\tau_i^D(0)+\tau_i^A(0)}{T_i}$
% 		\STATE $q_i$ = $max(0, RC_i^0 - (1-U^M)\dot (d_i(t_{cur}-d_1(t_{cur}))))$ 
% 		\STATE $U^M$ = $min(1.0, U^M+ \frac{d_i(t_{cur} - d_1(t_{cur}))}{RC_i^0-q_i})$
% 		\STATE $p$ = $p + q_i$
% 		\ENDFOR
% 		\STATE  $Slack(t_{cur}, d_1(t_{cur})) $ = $d_1(t_{cur}) - t_{cur} - p$
% 		\STATE \textbf{return} arg $\max_{s_k \in S_k}\{C_k^D(s_k)|C_k\}$
% 	\end{algorithmic}
% 	\normalsize
% \end{algorithm}

% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% \noindent
% \begin{theorem}
% If equation~\eqref{eq:schedulable} holds for $\tau$, then $\tau$ is schedulable by EDF-Aging
% \end{theorem}
% \begin{proof}
% \hb{proof here}
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% \end{proof}
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\
% ~\\~\\~\\

